Approximating Rectangles by Juntas and Weakly-Exponential Lower Bounds for LP Relaxations of CSPs

We show that for constraint satisfaction problems (CSPs), sub-exponential size linear programming relaxations are as powerful as $n^{\Omega(1)}$-rounds of the Sherali-Adams linear programming hierarchy. As a corollary, we obtain sub-exponential size lower bounds for linear programming relaxations that beat random guessing for many CSPs such as MAX-CUT and MAX-3SAT. This is a nearly-exponential improvement over previous results, previously, it was only known that linear programs of size $n^{o(\log n)}$ cannot beat random guessing for any CSP (Chan-Lee-Raghavendra-Steurer 2013). Our bounds are obtained by exploiting and extending the recent progress in communication complexity for "lifting" query lower bounds to communication problems. The main ingredient in our results is a new structural result on "high-entropy rectangles" that may of independent interest in communication complexity.

==> single-filet.tex <==
% !TEX root = maint.tex
%\newcommand{\Errora}{Errora}
%\newcommand{\Errorb}{Errorb}
\newcommand{\rnng}{\R_{\geq 0}}

\section{Introduction}
Translating a combinatorial problem over a discrete domain to a problem in continuous space has been an important concept in computer science over the last few decades; in this vein, linear programming relaxation is one of the most used techniques for algorithm design. In this work we prove limitations on the power of linear programs (LPs) as applied to \emph{constraint satisfaction problems} (CSPs).

Constraint satisfaction problems such as MAX-3SAT or MAX-3XOR or MAX-CUT are some of the most well-studied problems in approximation algorithms as well as combinatorial optimization. Here we show unconditional lower bounds for approximately solving CSPs by LPs. Informally, we show that for many CSPs such as MAX-3SAT, MAX-3XOR, or MAX-CUT, no LP of size $2^{n^{\Omega(1)}}$ can beat the \emph{trivial} approximation factor ($7/8$ for MAX-3SAT, $1/2$ for MAX-3XOR, $1/2$ for MAX-CUT); we also show similar results for vertex-cover. Previously, such lower bounds only applied to LPs of size at most $n^{\Omega((\log n)/(\log \log n))}$ \cite{CLRS13}.

The core of our result above is a new structural result about rectangles that has various applications in communication complexity in the context of \emph{lifting query} lower bounds to communication lower bounds.

\subsection{CSPs, Linear programming relaxations, Sherali-Adams hierarchy} \label{sec:lpforCSP}
A MAX-CSP (henceforth referred to only as CSP) is defined by a \emph{predicate} $P: \on^k \rightarrow \{0,1\}$. An instance of the CSP, $\cal{I}$, is defined by a collection of $k$-tuples of literals $C_1, C_2, \ldots, C_m$ on $n$ Boolean variables $(x_1, x_2, \ldots, x_n)$ \footnote{Throughout this article, we will use $\{-1,1\}$ to denote boolean inputs}. The algorithmic problem is to find an assignment to the variables $x = (x_1,\ldots,x_n)$ so as to maximize the number of satisfied constraints:

\begin{equation}\label{eq:cspdef}
\opt(\cal{I}) = \max_{x \in \on^n} \sum_{i=1}^m P(C_i(x)) \equiv \max_{x \in \on^n} \cal{I}(x),
\end{equation}
where we define $\cal{I}(x)  = \sum_{i = 1}^m P(C_i(x))$.

For example, MAX-CUT corresponds to the case where the predicate $P:\on^2 \to \zo$ is defined by $P(a,b) = (1 - ab)/2$ with instances corresponding to graphs.

Here we consider a broad-class of linear programming relaxations for CSPs obtained by \emph{linearizing} the objective function $\cal{I}(x)$. Formally, given a predicate $P$, and an integer $D$, we want:

\begin{definition}[Linearization of a CSP]
\begin{enumerate}
\item A vector $v_x \in \R^D$ for every $x \in \on^n$.
\item A vector $w_\cal{I} \in \R^D$ for every instance $\cal{I}$ of the CSP.
\item For every assignment $x$ and every instance $\cal{I}$, $\cal{I}(x) = \iprod{w_\cal{I},{v_x}}$.
\end{enumerate}
\end{definition}

Given a linearization as above, we can define a relaxation of the CSP as follows.  For a polytope $\cal{P} \subseteq \R^D$ with $\{v_x: x \in \on^n \} \subseteq \cal{P}$, we look at the linear program
$$\opt_{\cal{P}}(\cal{I}) = \max_{y \in \cal{P}} \iprod{w_\cal{I},{y}}.$$
Clearly, $\opt(\cal{I}) \leq \opt_{\cal{P}}(\cal{I})$. The \emph{complexity} or \emph{size} of the relaxation is defined as the number of facets (or inequalities) needed to describe the polytope $\cal{P}$.

\textbf{$(c,s)$-approximation.} We say that a relaxation $\cal{P}$ as described above, achieves an $\alpha$-approximation factor if for every instance $\I$, $ \opt_{\cal{I}} \geq  \alpha \opt_{\cal{P}}(\cal{I})$. More generally, we say that $\cal{P}$ achieves a $(c,s)$-\emph{approximation} if for all instances $\cal{I}$ such that $\opt(\cal{I}) \leq s$, $\opt_{\cal{P}}(\cal{I}) \leq c$.

\PRnote{ToDo: define relaxation as a sequence of polytopes?}

The above framework introduced in the work of \cite{CLRS13} generalizes the \emph{extended formulation} framework of Yannakakis \cite{Yan88} and its adaptation to approximation algorithms studied in \cite{BFPS15}.  Furthermore, LPs arising out of the Lovasz-Schriver (LS) \cite{LovaszS} or the Sherali-Adams \cite{SheraliA} hierarchies are captured within the this framework.

We prove that despite its apparent vast generality, when it comes to CSPs, general linear programs as above, and hence all extended formulations, are only as powerful as those obtained from the Sherali-Adams hierarchy:

\begin{theorem}\label{thm:maincsp}
There exist constants $0 < h < H$ such that the following holds. Consider a function $f:\mathbb{N} \to \mathbb{N}$. Suppose that the $f(n)$-round Sherali-Adams relaxation for a CSP cannot achieve a $(c,s)$-approximation on instances on $n$ variables. Then, no LP relaxation of size $n^{hf(n)}$ can achieve a $(c,s)$-approximation for the CSP on $n^H$ variables.
\end{theorem}

In conjunction with known lower bounds for Sherali-Adams relaxations \cite{cmm}, the above theorem yields the following corollary:
\begin{corollary}\label{cor:maincsp}
For every $\epsilon > 0$, there exist constants $c_\epsilon, c'_\epsilon$ such that the following holds. No LP relaxation of size less than $2^{n^{c_\epsilon}}$ can achieve a $(7/8 + \epsilon)$-factor approximation for MAX-3SAT. Similarly, no LP relaxation of size less than $2^{n^{c_\epsilon'}}$ can achieve a $(1/2+\epsilon)$-factor approximation for MAX-CUT.
\end{corollary}

\RMnote{Corollary for vertex cover?}
\pnote{add paragraph explaining significance: }\\
\RMnote{Also need to add proofs of these corollaries somewhere with appropriate citations to the $degree_+$/SA lower bounds.}

 The above results for CSPs are established through a more general claim on \emph{non-negative rank} of a class of matrices referred to as \emph{pattern matrices}. We explain this connection and results next.

\subsection{Lifting degree lower bounds to rank lower bounds}
In the seminal work introducing extended formulations, Yannakakis showed that the extended formulation complexity of an optimization problem is precisely the {\it non-negative rank} of the associated slack matrix.  In \cite{BFPS15}, this connection was subsequently extended to approximation by linear programs.  All known lower bounds on the size of extended formulations rely on this connection as do we.

\begin{definition}[Non-negative Rank]
Let $M$ be a non-negative matrix. The non-negative rank of $M$, denoted by $\nnr(M)$ is the least positive integer $r$ such that there exist non-negative rank $1$ matrices $M_1,\ldots, M_r$ such that $M = \sum_{i = 1}^r M_i$.
\end{definition}

Proving lower bounds on non-negative rank of specific matrices is often non-trivial; the first breakthrough was achieved by the work of \cite{FMPTdW15}. Before the work of \cite{FMPTdW15} there was no super-constant separation between the rank and non-negative rank of any explicit matrix.
\RMnote{I wrote the last sentence, but I am now no longer sure of this: what was the first gap?}

We give a tight characterization of the non-negative rank of a broad-class of matrices--\emph{pattern matrices}-- that were studied before in communication complexity \cite{razmckenzie,razborov,Sherstov11}. %We begin by recalling the definition of pattern matrices.

\begin{definition}[Pattern Matrix]  \label{def:lifted-matrix}
Fix positive integers $n$ and $q$.
%
Given functions $f: \on^n \to \R$ and $g : [q] \times [q] \to \on$, the composed function $f \circ g^{\otimes n} : [q]^n \times [q]^n \to \R$ is defined as,
\[ f\circ g^{\otimes n} (x,y) \defeq f \left(g(x_1,y_1),\ldots, g(x_n,y_n) \right) \mcom\]
where we have $x_i,y_i \in [q]$ for all $i \in [n]$.
%
The pattern matrix $M_f^g$ is the truth-table of the composed function $f \circ g^{\otimes n}$ expressed as a matrix, i.e., it is a matrix with rows and columns indexed by $[q]^n$ with,
\[M^{g}_f(x,y) \defeq f\circ g^{\otimes n} (x,y) \mper \]
\end{definition} %Observe that $\E[ M_f(x,y)] = 1$.

The function $g : [q] \times [q] \to \on$ is referred to as the {gadget function}.  Throughout this work, we will use the Boolean \emph{inner-product function} as the gadget $g$.  Specifically we will set $q = 2^b$ for $b \in \N$, identify $[q]$ with $\zo^b$ and define %  The gadget function $g$ is defined by %the $\on$ encoding of the following function,
$$\iproduct : \{0,1\}^b \times \{0,1\}^b \to \on \text{ given by } \iproduct(x,y) \defeq (-1)^{\oplus_{i=1}^b x_i y_i} \mper$$
%\[ \iproduct : \{0,1\}^b \times \{0,1\}^b \to \on \text{ given by } \mathsf{ip}(x,y) \defeq \oplus_{i = 1}^b x_i y_i \mper\]
With this choice of gadget function $g$, we will use $M^b_f$ to denote the pattern matrix $M_f^g$.  Furthermore, if the choice of $b$ is clear, we will drop the superscript and use $M_f$ to denote $M_f^b$.

Our main result characterizes the non-negative rank of pattern matrices $M_f$ by a corresponding measure of $f$ that we define next.

\begin{definition}[Juntas and Non-negative Degree]
A function $h:\on^n \to \mathbb{R}$ is a \emph{$d$-junta} if it only depends on at most $d$ coordinates. A function $h:\on^n \to \mathbb{R}_+$ is a \emph{conical} $d$-junta if it can be written as a non-negative linear combination of non-negative $d$ juntas.

For any $f:\on^n \to \mathbb{R}_+$, the non-negative degree of $f$, written as $\degp(f)$, is the least positive integer $d$ such that $f$ can be written as a conical $d$-junta.
\end{definition}
%\begin{definition}[$\epsilon$-Smooth Non-negative Degree] \label{def:degp}
%Let $f:\on^m \rightarrow \R^{+}$ be any non-negative function such that $\E[f] = 1$. The $\epsilon$-smooth non-negative degree of $f$, written as $\degp^{\epsilon}(f)$, is the least positive integer $d$ such that there exists a conical $d$-junta $h$, and an $\epsilon$-decaying function $e$ satisfying $|f(z) - (h(z)+e(z))| \leq \epsilon,$ for every $z \in \on^m$.
%\end{definition}
\ignore{
\begin{definition}[Non-negative Degree]\label{deg:degp}
Left $f:\on^m \rightarrow \R^{+}$ be a non-negative function such that $\E[f] = 1$. The non-negative degree of $f$, written as $\degp(f)$, is the least positive integer $d$ such that $f$ can be written as a conical $d$-junta.
\end{definition}}

We show that for any non-negative function $f$, the non-negative rank of $M_f$ is essentially characterized by the non-negative degree of $f$. Indeed, it is easy to check that
\begin{equation}\label{eq:easyubnnr}
\nnr(M^b_f) \leq \binom{n}{\degp(f)} \cdot 2^{b \cdot \degp(f)}.
\end{equation}


We show a nearly matching lower bound for $\nnr(M^b_f)$; specifically, we show that if small positive shifts of $f$ have\footnote{Note that $\degp(f+\eta) \leq \degp(f)$ for all $\eta > 0$.} high non-negative degree, then $\nnr(M_f)$ is correspondingly large.

%We show that for any non-negative function $f$ that cannot even be approximated by low-degree conical juntas, the corresponding matrix $M_f$ has a high non-negative rank. Since we work with an approximation for $f$ that works up to additive errors, we normalize $f$ so that $\E[f] =1$.
%The main technical contribution of this work is to show that the non-negative rank of the matrix $M_f$ can be lower bounded in terms of non-negative degree of $f-\epsilon$ and is encapsulated in the following theorem.

\begin{theorem}[$\nnr(M_f)$ vs $\degp(f)$]\label{thm:nnrlift}
There exist constants $1 \leq c,C $ such that the following holds. Let $f:\on^n \rightarrow \R^{+}$ be such that $\E[f] = 1$. Then, for all $\eta \geq c/n$ and $b \geq C(\log_2 n)$, $$\nnr(M^b_f) \geq  2^{\Omega( b \cdot \degp(f+\eta))}.$$ \label{thm:main-tech}
\end{theorem}
%
Note that by \eref{eq:easyubnnr}, for $b > \log n$, $\nnr(M^b_f)  \leq 2^{2b \cdot \degp(f)}$. Thus, the above theorem is tight up to constant factors (in the exponent) and working with $\degp(f+\eta)$.

\subsection{Previous work: Approximate non-negative rank versus non-negative rank}
The above result should be compared with similar results in \cite{GLMWZ15, LRS15} . Although they also obtain similar lifting theorems, a crucial difference is that they lower bound the \emph{approximate non-negative} rank of lifted matrices. For a non-negative matrix $M$, and $\eps > 0$, define the $\epsilon$-approximate non-negative rank as
$$\nnr^\epsilon(M) = \min\{\nnr(M'): \|M'-M\|_\infty \leq \epsilon \|M\|_\infty\}.$$

Clearly, $\nnr^\epsilon (M) \leq \nnr(M)$ for all $\epsilon > 0$. At a high-level, the previous works show lower bounds on $\nnr^\epsilon(M_f)$ (in terms of the \emph{approximate non-negative junta} degree of $f$). Similarly, while \cite{GLMWZ15} separate a separation between $\nnr^\epsilon, \nnr^\delta$ for some constants $0 < \epsilon < \delta < 1$, the resulting matrices have large rank. Such lifting theorems are not enough to obtain our applications to CSPs -- \prettyref{thm:maincsp}, \prettyref{cor:maincsp} -- as matrices arising in these applications in fact have small approximate non-negative rank (roughly $n^{O(\log(1/\epsilon))}$) and small rank. This was one of the main reasons why the previous works only obtained quasi-polynomial size lower bounds.

In fact, before our work, the best separation between $\nnr^\epsilon$, $rank$ and $\nnr$ was only quasi-polynomial. As a corollary of our results, we obtain subexponential separation for an explicit matrix:
\begin{theorem}
For all $\epsilon > 0$, there exist constants $0 < c_\epsilon, C_\epsilon$ such that the following holds. There exists an explicit non-negative matrix $M \in \R_+^{N \times N}$ such that $rank(M), \nnr^\epsilon(M) \leq (\log N)^{C_\epsilon \log \log N}$ and $\nnr(M) > \exp((\log N)^{c_\epsilon})$.
%$rank(M) < (\log n)^{C_\epsilon}$, $\nnr(M) > 2^{\bkets{\nnr^\epsilon(M) + rank(M)}^{c_\epsilon}}$.
\end{theorem}
\RMnote{Need to write down the proof somewhere.}

\subsection{Applications in Communication Complexity}
Analyzing lifted functions or pattern matrices has been a very useful tool in communication complexity over the last few years and our work builds on the techniques of \cite{GLMWZ15} who show lifting theorems for various \emph{rectangle-based} communication measures. Our main decomposition theorem, \prettyref{thm:maindecomp}, can be used to recover the main results of \cite{GLMWZ15}. Indeed, the main results of \cite{GLMWZ15} follow from a structural result about approximating \emph{rectangles} by \emph{juntas} -- an analogue of \prettyref{thm:mainjunta} that in turn follows easily from our decomposition theorem. For a more detailed comparison, see the discussion at the beginning of \prettyref{sec:decompalgorithm}. We believe that our decomposition theorem could lead to other such applications in future.
\section{Proof overview}

\subsection{Lifting $\degp$ lower bounds to non-negative rank}
% \begin{theorem}[$\nnr(M_f)$ vs $\degp(f)$, Theorem \ref{th:nnrlift} restated]
% There exist constants $0 < c,C $ such that the following holds. Let $f:\on^n \rightarrow \R^{+}$ such that $\E[f] = 1$. Then, for all $\eta \geq c/n$ and $M_f$ defined with blocksize $b \geq C \log_2 n$, $$\nnr(M_f) \geq  2^{\Theta( b \degp(f+\eta))}.$$ \label{thm:nnrliftrestated}
% \end{theorem}

The proof of \prettyref{thm:nnrlift} consists of two steps.  First, we show that if $\nnr(M_f)$ is small for a function $f$, then $f$ can be \emph{approximated} by a conical junta under a carefully chosen notion of {\it approximation}.  Second, we show that if $f$ can be so approximated by a conical junta, then $\degp(f+\eta)$ is small for $\eta \ll 1$.

Towards making this outline more precise, we begin by defining a notion of approximate conical juntas that plays an important role in our proofs. We first state some basic notations that we use throughout:

\begin{itemize}
\item For any function $f$, $\E[f]$ denotes the expectation of $f$ on the uniform distribution over its domain.
\item For any $x \in \on^n$ and $I \subseteq [n]$, we write $x_I$ to denote the projection of $x$ on to the coordinates in $I$.
\item A \emph{Boolean conjunction} $C:\on^n \to \R_+$ is defined by a subset $I \subseteq [n]$ of variables and $\alpha$ an assignment to the variables in $I$ by $C(x) = 2^{|I|} \cdot \1[x_I = \alpha]$. We say $C$ is a $d$-conjunction if $|I| \leq d$. Observe that we choose a non-standard scaling that satisfies $\E[C] = 1$.
\item For any $S \subseteq [n]$, the parity function $\chi_S(x) = \Pi_{i \in S} x_i$ for any $x \in \on^n$. Any function $f: \on^n \to \R$ has the \emph{Fourier expansion} $f(x) = \sum_{S \subseteq [n]} \hat{f}(S) \chi_S(x)$. The terms $\hat{f}(S)$ are the Fourier coefficients of $f$.
\end{itemize}
%First, we define the notion of $\epsilon$-decaying functions.
\begin{definition}[$\epsilon$-decaying functions]
For $0 < \epsilon < 1$, a function $h: \on^n \rightarrow \R$ is said to be $\epsilon$-decaying if $\E[h] = 0$ and for every $I \subseteq [n]$, $|\hat{h}(I)| \leq \epsilon^{|I|}.$
\end{definition}

\begin{definition}[$(\epsilon,\delta)$-approximate conical $d$-junta]
For $\epsilon,\delta \in (0,1)$, a function $f : \on^n \to \R^+$ with $\E[f] = 1$ is said to be an {\it $(\epsilon,\delta)$-approximate conical $d$-junta} if $f$ can be written as
\begin{equation}
f(z) = \sum_{i \in [N]} \lambda_i C_i(z) \cdot (1+ h_i(z)) + \gamma(z)
\end{equation}
for $d$-conjunctions $C_1,\ldots,C_N$, $\epsilon$-decaying functions $h_1,\ldots,h_N$,  $\lambda_1,\ldots, \lambda_N \in \rnng$ with $\sum_{i} \lambda_i < 1$, and a function $\gamma:\on^n \to \rnng$ such that $\E[\gamma] \leq \delta$. %\RMnote{Why is this condition on $\lambda_i$ necessary? Don't we always also get $\gamma$ to be positive? If so, this is redundant}\footnote{In this work, all the approximations we construct will have $\gamma$ to be a non-negative function.}
\end{definition}

Notice that the approximation by conical-juntas has two distinct error terms, the multiplicative errors due to the $\epsilon$-decaying functions $\{h_i\}$ and the additive error in the form of $\gamma$.

The first step in proving \prettyref{thm:nnrlift} is the following lemma saying that if $\nnr(M_f)$ is small, then $f$ is an approximate conical $d$-junta for small $d$.% low-degree approximate conical junta as above. %Now, we are ready to state our key lemma that approximates functions $f$ with small $\nnr(M_f)$ as approximate conical juntas.

\begin{lemma}[Non-negative rank to Approximate Conical Juntas] \label{lem:approx-conical}
There exists a constant $\alpha_1 \geq 1$ such that the following holds. Let $f:\on^n \to \R_+$ with $\E[f] = 1$ and let $r = \nnr(M_f^b)$ for $b \geq \alpha_1 \log_2 n$. Then, $f$ is a $(2^{-b/2},2^{-bd/\alpha_1})$-approximate conical $d$-junta for all $d \geq \alpha_1 (\log r)/b$.
\end{lemma}
\ignore{There exists a constant $\alpha_1 > 0$ such that the following holds:
Suppose $r = \nnr(M_f)$, then $f$ is a $(\epsilon,\delta)$-approximate conical $d$-junta with $\epsilon = 2^{-0.5 b}$, $\delta = r \cdot 2^{-bd}$ and  $d  = \frac{\alpha_1 \cdot \log{r}}{b}$.
\end{lemma}}

We defer the sketch of the proof of the lemma to the next section and continue with our outline of the proof of \prettyref{thm:nnrlift}.

Given the above lemma, the final step in proving \prettyref{thm:nnrlift} is to show a connection between $\degp(f)$ and $(\epsilon,\delta)$-approximation by conical juntas.  Specifically, we show a certain {\it robustness} of the class of conical juntas: if a function $f$ is an $(\epsilon,\delta)$-approximate conical $d$-junta for sufficiently small $\epsilon$ and $\delta$, then the function $f+\eta$ is an exact conical $8d$-junta for a small constant $\eta$.

\begin{lemma} \label{lem:approx-to-exact}
Suppose $f : \on^n \to \rnng$ with $E[f] < 1$ is a $(\epsilon,\delta)$-approximate conical $d$-junta for $\epsilon < 1/n^4$ and $\delta < 1/n^{8d}$ then \[ \degp\left(f+\frac{1}{n}\right) < 8d\]
\end{lemma}

\prettyref{lem:approx-conical} and \prettyref{lem:approx-to-exact} together imply \prettyref{thm:nnrlift} almost immediately by setting the parameters appropriately; see \prettyref{sec:nnrlift}.%  The details are as follows.

%\begin{proof}[Proof of \prettyref{thm:nnrlift}]
%\PRnote{need to pick large enough b and combine previous two lemmas}
%\end{proof}

We defer the proof of \prettyref{lem:approx-to-exact} to \prettyref{sec:approx-to-exact}.  In what follows, we sketch the key ideas underlying the proof of \prettyref{lem:approx-conical}.

% \pnote{marked for deletion:
% The proof of our lower bounds for CSPs, \tref{thm:maincsp}, \cref{cor:maincsp}, can be broken down into four modular steps:
% \begin{enumerate}
% \item Reduce proving lower bounds for CSPs to proving lower bounds on the rank of lifted matrices $M_f$ as in \tref{th:nnrlift}.
% \item Proving Lemma \ref{lem:nnrlifted} using the strong junta theorem as in Lemma \ref{lem:mainjunta}.
% \item Proving \tref{th:juntas} using the decomposition result \tref{thm:maindecomp}.
% \item Prove the decomposition theorem.
% \end{enumerate}

% We explain each of these steps next. Much of the technical work goes into proving \tref{thm:maindecomp}. The proof of the first step is based on the ideas in \cite{CLRS13}. The main ingredients in the second step are the junta approximation theorem and some properties of the dual to the Sherali-Adams LP. The third step uses the main decomposition result along with an observation about $\bd$ densities noted first in \cite{GLMWZ15}.
% }

\subsection{Approximating Rectangles by Conical Juntas}
We now sketch the proof of \prettyref{lem:approx-conical}. To do so, we need the following basic definition\footnote{We work with densities (instead of equivalently working with probability density functions or just non-negative functions) as  keeping track of errors is cleaner under this normalization.}.
\begin{definition}[Density]
A function $p: [q]^{n} \rightarrow \R^{+}$ is said to be a density if $\E[ p(x) ] = 1.$ A density $p$ defines a corresponding random variable $X$ on $[q]^n$ where $Pr[X= x] = p(x) \cdot q^n$. We denote $X \sim p$ this random variable.
\end{definition}

Recall the statement of the lemma: we have a density $f$ on $\on^n$ such that $M_f$ has small non-negative rank and we want to show that $f$ is a low-degree approximate conical junta. Let $\nnr(M_f) = r$.  By definition, $M_f = \sum_{i \in [r]} M_i$ where each $M_i$ is a non-negative rank one matrix; further, by appropriate normalization, we can assume that $M_i = \lambda_i u_i v_i^\dagger$, where $u_i,v_i$ are densities on $[q]^n$ and $\lambda_i > 0$. This decomposition of the matrix $M_f$ into non-negative rank $1$ matrices $\{M_i\}$, yields a corresponding decomposition of the function $f$ into a sum of non-negative functions, one corresponding to each rank one matrix $M_i$.

Formally, let us denote by $G :[q]^n \times [q]^n \to \on$ the function $G \seteq g^{\otimes n}$.  By definition, the entries of the matrix $M_f$ are given by $M_f(x,y) = f\left( G(x,y) \right)$.  For $z \in \on^n$, let $(X,Y) \sim  G^{-1}(z)$ denote a uniformly random pair chosen from the set of pairs $G^{-1}(z) \subseteq [q]^n \times [q]^n$.  With this notation,
\begin{equation}\label{eq:intromainjunta1}
 f(z) = \E_{(X,Y) \sim G^{-1}(z)} M_{f}(X,Y) = \sum_{i \in [r]} \E_{(X,Y) \sim G^{-1}(z)} \left[ M_i(X,Y) \right] = \sum_{i \in [r]} \lambda_i \E_{(X,Y) \sim G^{-1}(z)}\sbkets{u_i(X) v_i(Y)}\mper
 \end{equation}

Borrowing terminology from communication complexity, we will refer to the rank one matrices $u_i v_i^\dagger$ as {\it rectangles}.  In order to approximate the function $f$ by a conical junta, it suffices to approximate the terms corresponding to each {\it rectangle} by a conical junta.  We exhibit such an approximation for all {\it large rectangles}.

\ignore{%At the cost of slight abuse of notation, we will use entropy for what is usually known as min-entropy.

 For the sake of concreteness, let us suppose
\[M_i(x,y) = \lambda_i \cdot u_i(x) \cdot v_i(y)\]
where $u_i, v_i : [q]^n \to \R^+$ are densities.

Then, from the above arguments, we get
$$f(z) = \sum_{i=1}^r \lambda_i \E_{(x,y) \sim G^{-1}(z)}[u_i(x) v_i(y)].$$}
%non-negative functions satisfying $\E_x[u_i(x)] = \E_{y}[v_i(y)] = 1$ and $\lambda_i$ is a non-negative constant.  Here the functions $u_i$ and $v_i$ are normalized to be densities over $[q]^n$.

Towards this end, for two densities $u,v$ on $[q]^n$, define $Acc_{u,v}:\on^n \to \R_+$ by
\begin{equation}\label{eq:defacc}
Acc_{u,v}(z) = \E_{(X,Y) \sim G^{-1}(z)}[u(X) v(Y)].
\end{equation}


Note that $\E[Acc] = \E[u(x) v(y)] = 1$. Thus, $Acc$ is a density on $\on^n$. Indeed, it is easy to check that $Acc_{u,v}$ is the density of the random variable $G(X,Y)$ for $X \sim u$ and $Y \sim v$ ($X,Y$ independent). Using this definition in \prettyref{eq:intromainjunta1}, we get
$$f(z) = \sum_{i=1}^r \lambda_i \cdot Acc_{u_i,v_i}(z).$$

This motivates the study of functions $Acc_{u,v}$ for rectangles. Indeed, structural results characterizing such functions form the core of previous results on pattern matrices \cite{sherstov, GLMWZ15}. We show that functions $Acc_{u,v}$ as above are \emph{simple} when the rectangle $u\times v$ is \emph{large}. To formalize this we need the notion of \emph{min-entropy}.

\begin{definition}[Min-Entropy]
For a density $u$ on $[q]^{n}$, the \emph{min-entropy} of $u$, $H_\infty(u)$, is defined by\footnote{Note that this is the same as the more standard definition of $\min_{x \in \on^n} \log(\pr[X=x])$ where $X \sim u$.}\footnote{Throughout this work, all logarithms are to the base $2$.} $$H_{\infty}(u) = \min_{x \in \on^n} \log {(q^n/u(x))}.$$
\end{definition}

For intuition, it is helpful to think of the special case where the densities $u_i, v_i$ correspond to uniform distributions over some subsets $U_i, V_i$ of $[q]^n$ respectively.  The rectangle $M_i$ is said to be large, if the sets $U_i$ and $V_i$ are both {\it large}, of size at least $q^{n}/2^{C}$ for $C << n$. More generally, the rectangle $M_i$ is large if the distributions $u_i,v_i$ each have min-entropy at least $n \log{q} - C$. We will refer to $C$ as the {\it min-entropy deficiency}.

Since $M$ is the sum of $r$ rectangles, one can argue that it is approximated by {\it large} rectangles whose min-entropy deficiency is at most $O(\log{r})$.  The contribution from all the {\it small} rectangles can be included into the additive error term $\gamma(z)$ in the approximation for $f$.  The main work lies in showing that every {\it large rectangle} is approximated by conical juntas.  %can be expressed as a perturbation of a non-negative junta of degree $d \approx t/b$. \pnote{say something meaningful about the multiplicative error and why it shows up and is important.}

\begin{theorem}[Junta Approximation]\label{thm:mainjunta}
There exists a constant $\alpha_2 \geq 1$ such that the following holds. Let $u,v$ be densities over $[q]^n$ with $q =2^b$ such that $H_{\infty}(u)+ H_{\infty}(v) \geq 2b(n-t)$. Then, for all $b \geq \alpha_2 \log n$ and $d \geq \alpha_2 t$, $Acc_{u,v} \on^n \to \rnng$ is a $(2^{-0.5b},(2^{-0.5b})^d)$-approximate conical $d$-junta.

%and $\epsilon = 2^{-0.5b}$, $Acc_{u,v}:\on^n \to \R_+$ is a $(\epsilon,\epsilon^d)$-approximate conical $d$-junta.
\ignore{There exist $d$-conjunctions $C_1, C_2, \ldots, C_N:\on^n \to \R_+$, $\epsilon$-decaying functions $h_1,\ldots,h_N:\on^n \to \R$, a density $\gamma:\on^n \to \R_+$, and non-negative weights $\lambda_1,\ldots,\lambda_N, \lambda_{err} \geq 0$ such that
$$A_{p,q}(z) = \sum_{i=1}^N \lambda_i C_i(z) (1 + h_i(z)) + \lambda_{err} \gamma, $$
where $\sum_{i=1}^N \lambda_i + \lambda_{err} = 1$, and $|\lambda_{err}| \leq \epsilon^d$.}
\end{theorem}

\cite{GLMWZ15} also has show a similar, but weaker, junta approximation theorem. In the present context, they essentially show that $Acc_{u,v}$ can be approximated as $Acc_{u,v}(z) = (1\pm 2^{-\Omega(b)}) \cdot h(z) \pm 2^{-\Omega(bd)}$ where $h$ is a conical $d$-junta. Note that the multiplicative error is only of the order $2^{-\Omega(b)}$ and this was an important bottleneck in using their results for proving a lifting theorem for non-negative rank as in \prettyref{thm:nnrlift}.  In comparison, we get exponentially small error in terms of approximate conical $d$-juntas. The latter is in fact stronger, and a straightforward extension of our arguments can be used to recover the corresponding statement of \cite{GLMWZ15}.
\RMnote{Please check this wording.}
%\RMnote{It is important to compare with GLMWZ and similar structural results used in pattern matrices. Otherwise, no one will see why old stuff did not work for non-negative rank.}


%  Now we will outline the proof of approximation by conical juntas.
%  Suppose M_f has rank r, then M = \sum_i M_i where each M_i is rank 1.  now, we can write f as sum of rectangle
% since there are very few rectangles, almost all of them are large, i.e., ..
% this reduces the question to can we approximate the function from a rectangle by a \epsilon,\delta-approximate conical junta

\subsection{Decomposing High-Entropy Distributions}

The proof of \prettyref{thm:mainjunta} relies on a crucial decomposition lemma for high-entropy distributions that may be of independent interest. Let $u,v$ be two densities over $[q]^n$ with min-entropy at least $(n-C) \cdot \log{q}$ for some $C \ll n$ and let $X \sim u, Y \sim v$ be sampled independently.

%Let $X,Y$ denote independent random variables over $[q]^n$ sampled from $u$ and $v$ respectively.

%Let $X,Y$ be two independent distributions over $[q]^{n}$ with very high min-entropy: $H_\infty(X), H_\infty(Y) \geq (nb) - C$. That is, $X,Y$ have min-entropy \emph{deficiency} at most $C$. Such distributions arise commonly in communication complexity---they correspond to large rectangles. We would like to study the product distribution $X \times Y$ on $(\zo^b)^n$ and decompose them into distributions with more structure.

A particularly simple class of high min-entropy distributions are those where a subset of $C$ coordinates of $X$ are fixed, while the rest are uniformly random. That is, for some set $I \subseteq [n]$ with $|I| \leq C$, $X_I$ is a fixed string whereas $X_{[n]\setminus I}$ is uniformly random over $[q]^{[n] \setminus I}$. Similarly, $Y$ could satisfy a similar property for a set $J \subseteq [n]$ with $|J| \leq C$. An especially desirable scenario is one where $X,Y$ are \emph{aligned} in the sense that $I=J$. For such aligned distributions, the random variable $Z = g^n(X,Y) \in \on^n$ is such that $Z_I$ is fixed while $Z_{\overline{I}}$ is uniformly random.  In other words, the probability density of $Z$ is a $C$-junta depending only on $I$.

We will show that as long as $X,Y$ have high min-entropy, the product distribution $X \times Y$ can be decomposed into distributions that are essentially as simple and aligned as in the above discussion.

To this end, we next introduce the notion of \emph{blockwise-dense} distributions; they were first defined in \cite{GLMWZ15} and play a crucial role here.
\begin{definition}
A distribution $X$ on $[q]^{n}$ is \emph{\bd} if for every $I \subseteq [n]$, $H_\infty(X_I) \geq 0.8 \cdot \log q \cdot |I|$. We say a density $u$ on $[q]^n$ is \bd if $X \sim u$ is \bd.
\end{definition}

\PRnote{use blocks or coordinates over q???}
\RMnote{I think coordinates is better when dealing with $q$.}
\begin{definition}
A distribution $X$ on $[q]^{n}$ is a $d$-\cbd (``conjunctive blockwise-dense'') distribution if for some set of coordinates $I \subseteq [n]$, $|I| \leq d$, $H_\infty(X_I) = 0$ and for every $J \subseteq [n] \setminus I$, $H_\infty(X_J) \geq 0.8 \cdot \log{q} \cdot |J|$. We refer to $d$ as the \emph{degree} of the \cbd distribution, and the set of blocks $I$ as the {\it fixed} blocks. We say two $d$-CBD distributions $X,Y$ on $[q]^{n}$ are aligned if the \emph{fixed} blocks $I$ are the same in both.

Analogously, we say two densities $u,v$ over $[q]^n$ are aligned $d$-\cbd if the random variables $X,Y$ are aligned $d$-\cbd distributions for $X \sim u, Y \sim v$.
\end{definition}

The technical core of our results is the following lemma stating that any two independent high-entropy densities $u,v$ over $[q]^n$ can be approximated by a convex combination of aligned $d$-\cbd densities for small $d$. The error of the approximation will depend on the entropy deficiency of $u  \otimes v$ and the degree of the $\cbd$ distributions used in the approximation.

%Our core lemma states that any two independent high-entropy distributions $X,Y$ over $[q]^n$ can be approximated by a convex combination of aligned \cbd distributions. The error of the approximation will depend on the entropy deficiency of $X \times Y$ and the degree of the $\cbd$ distributions used in the approximation.

\begin{theorem}\label{thm:maindecomp}
There exists a constant $c \geq 1$ such that the following holds. For $n \geq 1$ and $q \geq n^c$, let $u,v$ be two densities on $[q]^n$ with $H_\infty(u) + H_\infty(v) \geq 2(n-t) \cdot \log{q}$. Then, for all $d \geq ct/(\log q)$, the product density $u \otimes v$ on $[q]^n \times [q]^n$ can be written as a convex combination of densities $u_1 \otimes v_1, u_2 \otimes v_2,\ldots, u_N \otimes v_N$, and $\gamma_{error}$, i.e., 
$u \otimes v = \sum_{i=1}^N \lambda_i u_i \otimes v_i + \lambda_{error} \gamma_{error}$, such that
\begin{itemize}
\item $0 \leq \lambda_1,\ldots,\lambda_N, \lambda_{err} \leq 1$, $\sum_{i=1}^N \lambda_i + \lambda_{err} = 1$.
\item $|\lambda_{err}| <  q^{-\Omega(d)}$.
\item For every $i \in [N]$, $X_i \sim u_i$, $Y_i \sim v_i$ are aligned $d$-\cbd distributions.
\end{itemize}
\end{theorem}

\ignore{
\begin{theorem}\label{thm:maindecomp}
%There exists a constant $c > 0$ such that the following holds.
Let $X,Y$ be two independent distributions over $[q]^{n}$ with $H_\infty(X) + H_\infty(Y) \geq 2n \cdot \log{q} - t$. Then, $X\times Y$ can be written as a convex combination of distributions $X_1 \times Y_1,\ldots,X_N \times Y_N , E$ over $[q]^{n} \times [q]^{n}$, i.e., $X \times Y = \sum_{i=1}^N \lambda_i X_i \times Y_i + \lambda_{err} E$, such that
\begin{itemize}
\item $0 \leq \lambda_1,\ldots,\lambda_N, \lambda_{err} \leq 1$, $\sum_{i=1}^N \lambda_i + \lambda_{err} = 1$.
\item $|\lambda_{err}| < 2^{t} (d q^{-0.05})^d$.
\item For every $i \in [N]$, $X_i, Y_i$ are aligned $d$-\cbd distributions.
\end{itemize}
\end{theorem}}

\prettyref{thm:mainjunta} follows easily from the above using some ``extractor''-like properties (cf.~Fact \ref{fact:ipextractor}) of the inner-product function $\iproduct$. We defer the details of the proof of the theorem to the corresponding section.
%\PRnote{add a lemma saying, d-CBDs with inner product gadget give epsilon decaying conical juntas.}

\subsection{Organization}
We present the proof in a top-down manner: We first prove \prettyref{thm:nnrlift} assuming \prettyref{thm:mainjunta}. We then prove \prettyref{thm:mainjunta} assuming \prettyref{thm:maindecomp} (this is almost immediate). Finally, we prove \prettyref{thm:maindecomp}.

\section{Preliminaries}
We describe some basic notation that we use throughout\footnote{To have all notations together, some are repeated from the introduction.}.
\subsection{Basic Notation}
\begin{enumerate}
\item $\P_d^n$ denotes the collection of all polynomials of degree at most $d$ on $n$ variables on $\on^n$.
\item $\1(E)$ is the indicator for the event $E$ normalized to have mean $1$. That is, $\1(E)$ is $0$ when $E$ doesn't happen and $1/\Pr[E]$ when $E$ happens.
\item For any function $f$, $\E[f]$ denotes the expectation of $f$ on the uniform distribution over its domain.
\item For matrices $M$, $\E[M]$ denotes the expectation of $M(x,y)$ under $x,y$ being uniformly random indices for its rows and columns.
\item For any $x \in \on^n$ and $I \subseteq [n]$, we write $x_I$ to denote the projection of $x$ on to the coordinates in $I$.
\item A \emph{Boolean conjunction} $C:\on^n \to \R_+$ is defined by a subset $I \subseteq [n]$ of variables and $\alpha$ an assignment to the variables in $I$ by $C(x) = 2^{|I|} \cdot \1[x_I = \alpha]$. We say $C$ is a $d$-conjunction if $|I| \leq d$. Observe that we choose a non-standard scaling that satisfies $\E[C] = 1$.
%\item A \emph{Boolean conjunction} $C:\on^n \to \R_+$ is defined by a subset $I \subseteq [n]$ of variables and $\gamma$ an assignment to the variables in $I$, and is the mean $1$ indicator $\1(x_I = \gamma).$ Observe that we choose a non-standard scaling that satisfies: $\E[C] = 1$ for any conjunction $C$ on $\on^n.$
\item For any $S \subseteq [n]$, the parity function $\chi_S(x) = \Pi_{i \in S} x_i$ for any $x \in \on^n$. Any function $f: \on^n \to \R$ has a Fourier expansion: $f(x) = \sum_{S \subseteq [n]} \hat{f}(S) \chi_S(x)$. The terms $\hat{f}(S)$ are the Fourier coefficients of $f$.


\end{enumerate}
\ignore{
\subsection{Probability}
\begin{definition}[Density]
A function $p: \on^{n} \rightarrow \R^{+}$ is said to be a density if $\E[ p(x) ] = 1.$
\end{definition}

%At the cost of slight abuse of notation, we will use entropy for what is usually known as min-entropy.
\begin{definition}[Min-Entropy]
For a density $p$ on $\on^{n}$, the \emph{min-entropy} of $p$, $H_\infty(p)$, is defined by  $$H_{\infty}(p) = \min_{x \in \on^n} \log {(2^m/p(x))}.$$
\end{definition}}


% \ignore{I don't think we need any additional discussion of gadgets, commented out:
% \subsection{Gadgets}
% Key ingredient to the transformation between a $n$ bit function $f$ and the corresponding lifted matrix $M_f \in \on^{bn} \times \on^{bn}$ is a \emph{gadget} that we briefly discussed in the introduction. We note down some key definitions here.

% A gadget $g: \on^{b} \times \on^b \rightarrow \on$ is just a function that maps a pair of $b$ bit strings into a single bit. We can use $g$ to product a function that operates on $n$ disjoint pairs of $b$ bit strings and outputs an $n$ bit string. In this context, we will think of any string in $\on^{bn}$ as an object of the form ${\on^{b}}^{\otimes n}$ and for any $x \in \on^{bn}$, write $x^i$ for the $i^{th}$ block of $b$ bits. We can then define $g^{\otimes n}: {\on^{b}}^{\otimes n} \times {\on^{b}}^{\otimes n} \rightarrow \on^n$ such that for any $x,y$, the $i^{th}$ bit of $g^{\otimes n}(x,y) = g(x^i, y^i).$

% We will work with the Boolean inner product gadget in this paper: $g(x,y) = \Pi_{i =1}^b (1+x_i)(1+y_i)$ and when not explicitly noted, $g$ will always denote the Boolean inner product function on pairs of $b$ bit strings.


% \subsection{Lifted Matrices}

% For any function $f: \on^n \rightarrow \R$, we can use a $b$ bit gadget $g$ to obtain a $f$-lifted matrix $M_f \in \on^{bn} \times on^{bn}$ as defined in the introduction: for any $x,y \in \on^{bn}$, $M_f(x,y) = \lambda \cdot f( g^{\otimes n}(x,y)),$ where $\lambda$ is chosen to ensure that $\E[M_f] = 1.$
% }



\subsection{Sherali-Adams Linear Programming Relaxations}
Our results relate arbitrary linear programming relaxations for CSPs to the Sherali-Adams hierarchy. We discuss the latter class of linear programs next. We begin with the definition of a {\it degree $d$ pseudo-expectation}

% \footnote{\pnote{no need for this foot note,delete it?} While there's no confusion in the present context, the term \emph{pseudoexpectation} is more often used in connection with the Sum of Squares SDP hierarchy where in addition to the constraints in Definition \ref{def:pE}, it satisfies the positive semidefiniteness constraint.}

\begin{definition}[Sherali-Adams Pseudoexpectation] \label{def:pE}
A degree $d$ Sherali-Adams pseudoexpectation, $\pE$, is a linear operator on the space of degree at most $d$ polynomials, $\P_d^n$, such that \begin{enumerate}
\item For every non-negative $p \in \P_d^n$ that depends on only $d$ variables, $\pE[p] \geq 0,$ and
\item $\pE[\1] = 1.$
\end{enumerate}
\end{definition}
%
Since $\pE$ is a linear, it is completely specified by its values on multilinear polynomials, in particular by the values $\pE[\chi_{S}(x)]$ for $S \subseteq [n]$, $|S| \leq d.$

Sherali-Adams linear programming relaxations can be equivalently described using a collection of probability distributions over local assignments. The above view is more convenient for us. We refer the reader to \cite{CLRS13journal} for a detailed discussion.

% \pnote{commenting this out:
% It is not hard to show that $\pE$ of Definition \ref{def:pE} is equivalently described by a collection of local probability distributions $\mu_S$, one for every $|S| \leq d$, $S \subseteq [n]$ such that for every $p \in \P_d^n$ that depends only on variables $x_i$ such that $i \in S$, $\pE[p] = \E_{\mu_S}[p].$
% }

The degree $d$-Sherali-Adams linear programming relaxation for a CSP solves the following optimization problem. Given an instance $\I$ of a $k$-ary CSP, we can canonically encode it as a polynomial of degree $k$ $P_\I:\on^n \to [0,1]$ such that $P_\I(x) = \I(x)$ for all assignments $x \in \on^n$. Then, the degree $d$-Sherali-Adams relaxation is

 \begin{equation} \max_{\pE} \pE[ P_\I(x)], \label{eq:SA-def} \end{equation}
where $\pE$ ranges over all degree $d$ Sherali-Adams pseudoexpectations. We define $\SA_d(\I)$ as the value of the the optimization problem \eqref{eq:SA-def}.
%
The above optimization problem can be solved using a linear program on $n^{O(d)}$ variables and constraints. Note that $\opt(\I) \leq \SA_d(\I)$.% for any $d \geq k.$

\paragraph{Sherali-Adams LP and Non-negative Degree:}
Linear programming duality gives an elegant characterization of the performance of Sherali-Adams LP on a CSP in terms of non-negative degree.

\begin{fact}[Sherali-Adams value and Non-negative Degree \cite{CLRS13}] \label{fact:savaldegp}
Let $P:\on^k \to \zo$ be a predicate and $\I$ be an instance of $CSP(P)$. Then, $\SA_d(\I) \leq c$ if and only if $\degp(c-\I) \leq d$.%Let $\I$ be an instance of CSP(P) with $\opt(\cal{I}) = s.$ The degree $d$-Sherali-Adams linear program achieves a value $c$ for $\I$ if and only $\degp(c-\I) \leq d.$
\end{fact}

\section{Non-negative Rank and LP Lower Bounds for CSPs}

In this section, we show that proving a lower bound on the size of any linear program for CSP(P) reduces to proving non-negative rank lower bound on a pattern matrix $M_f$ for an appropriate choice of $f$. Formally, the goal of this section is to show:

\begin{lemma}[LP Lower Bounds from Pattern Matrices] \label{lem:lplb-via-pattern}
Let $0 < s < c \leq 1$ and let $\Lambda:\on^k \to \zo$ be a predicate and let $\I^*$ be an instance of $CSP(\Lambda)$ on $n$ variables such that $\opt(\I^*) \leq s$ and let $f(x) = c- \I^*(x)$.
%Suppose for some positive integer blocksize $b$, the lifted matrix $M_f$ for $f(x) = c-\I(x),$ satisfies $\nnr(M_f) \geq R.$ Then, for $\eta = \Theta(1/2^bn)$ and
For all $g: [q] \times [q] \to \on$,  any linear programming relaxation of CSP(P) that achieves $(c,s)$-approximation on instances with $q \cdot n$ variables, has size at least $R \geq \Omega(\nnr(M^g_f)).$
\end{lemma}

The above lemma is an easy consequence of the characterization of size of linear programs  for CSPs \cite{CLRS13,Yan88}.
\PRnote{it is easier to state a lower bound result for lp size, than a characterization.  for lower bound, it is sufficient to define the matrix for plantings of an instance, whereas for characterization, one needs to define a single matrix for all instances.  I am going to state the characterization, may be we can scale back later}
%
Towards stating the characterization, let us fix a CSP $\Lambda$.  For $n \in \N$ and $s \in [0,1]$, let $\Lambda^s_n$ denote the family of all instances of the CSP on $n$ variables with $\opt(\cI) \leq s$.  With these definitions, we are ready to state the characterization.
\begin{fact} \cite{CLRS13} \label{fact:lpsize}
The size of the smallest linear program that $(c,s)$-approximates a CSP $\Lambda$ on instances with $n$ variables is $\Theta(\nnr(\cM_{n,s}))$ where the matrix $\cM_{n,s} : \Lambda^s_n \times \on^n \to \R$ is defined as
\[  \cM_{n,s}(\cI,x) \defeq c- \cI(x) \mper\]
\end{fact}
\PRnote{no reference for the above fact :(}
%\[\cF^s_n \defeq \{ \cI | \cI \text{ instance on } n \text{ variables with } \opt(\cI) \leq s \}\]

To prove \prettyref{lem:lplb-via-pattern}, we will show that $M_f^g$ is a sub-matrix of $\cM_{q \cdot n,s}$, and therefore $\nnr(\cM_{q \cdot n,s}) \geq \nnr(M_f)$.  By \prettyref{fact:lpsize}, this implies that the size of any LP that $(c,s)$-approximates the CSP on instances with $q \cdot n$ is at least $\nnr(M_f)$.  Hence, \prettyref{lem:lplb-via-pattern} is an immediate consequence of the following.

\begin{lemma}
Let $\I^{*}$ be an instance of CSP on $n$ variables such that $\opt(\I^*) = s$ and let $f(x) = c- \I^*(x)$.  Let $g: [q] \times [q] \to \on$ be a gadget function. Then, $M_f^{g}$ is a sub-matrix of $\cM_{q \cdot n, s}$.
\end{lemma}
\begin{proof}
%Let $g : [] \times \on^b \to \on$ denote the gadget function used to define $M_f^{b}$.
%
For $\alpha \in [q]$, define its \emph{$g$-encoding} $g \circ \alpha \in \on^{q}$ consisting of the truth-table of the function $g \circ \alpha : \beta \to g(\alpha,\beta)$.  Specifically, if we index the coordinates of $g \circ \alpha$ with $\beta \in [q]$, then $(g \circ \alpha)_{\beta} \defeq g(\alpha,\beta)$.  Similarly for $x \in [q]^{n}$, define $\tilde{x} \in \on^{q \cdot n}$ by setting $ \tilde{x}_i \seteq g \circ x_i$.

For each $y \in [q]^n$, we create an instance $\cI_y$ on $N = q \cdot n$ variables.  We will index the variables of $\cI_y$ by $[n] \times [q]$ and denote them by $\{z_{i,\beta} | i \in [n], \beta \in [q] \}$.  The instance $\cI_y$ is obtained by planting the instance $\I^*$ on the subset of variables $\{z_{1,y_1},\ldots,z_{1,y_n}\}$.

By definition of the matrices $\cM$ and $M_f^g$, we conclude that for any $x,y \in [q]^n$,
\begin{align*}
\cM_{q \cdot n, s}(\cI_y, \tilde{x}) & = c - \cI_y(\tilde{x}) \mcom\\
& = c - \cI^*\left( \tilde{x}_{1,y_1},\ldots, \tilde{x}_{1,y_n} \right) \mcom\\
& = c - \cI^* \left( (g \circ x_1)_{y_1},\ldots, (g \circ x_n)_{y_n} \right) \mcom \\
& = c - \cI^* \left( g(x_1,y_1),\ldots, g(x_n,y_n) \right) = f(g^n(x,y))\mcom \\
& = M_{f}^g(x,y) \mper
\end{align*}
Therefore, the matrix $M_{f}^g$ is a sub-matrix of $\cM_{q.n,s}$ as desired.
\end{proof}

\RMnote{Prove Theorems 1.2, Cor 1.3, 1.8 here. Basically need references.}


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \iffalse
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%COMMENTED OUT COMMENTED OUT
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% The proof of this lemma is simple. We first use the random planting idea (first employed by \cite{CLRS13} and then later by \cite{LRS15}) to obtain a \emph{random planting matrix} $M$ such that any linear programming relaxation for CSP(P) of size $R$ that achieves a $(c,s)$-approximation satisfies $R \geq \nnr(M).$
% %
% Then, we show that $M_f$ is a sub-matrix  of $M$ and therefore $\nnr(M) \geq \nnr(M_f).$ This completes the proof.

% We now describe the two claims above in more detail.  In the following, fix an instance $\I^{*}$ such that $\opt(\I^*) = s$, and let $f(x) = c - \I^{*}(x)$.
% %In the following, fix the hard instance $\I^{*}$ for  $d = f(n)$-degree Sherali-Adams linear programming relaxation of CSP(P) - i.e. $\opt(\I^{*}) = s$ while $\SA_d(\I^{*}) \geq c$. We also fix the ``slack'' function $f = c-\I^{*}$ on $\on^n.$

% \subsection{Random Planting Matrix}
% We begin by setting up some notation to talk about the random planting matrix that we will define. Let $m = 2^b n$ for some positive integer parameter $b$. We define the \emph{selection} function - this function takes input an index for each of the $n$ blocks and a $m$ bit string and outputs the $n$ bit string obtained by choosing the single bit pointed by the index from each block. Formally,

% \newcommand{\ind}{\mathsf{ind}}
% \begin{definition}
% Let $b,n$ be positive integers and $m = 2^bn$. The selection function $s:(\{-1,1\}^b)^{n} \times \on^{m} \rightarrow \on^n$ is defined so that for any $x \in \on^n$ and $\ind \in (\{-1,1\}^b)^{n}$ and $i \in [n]$, $$s(\ind,x)_i = x_{2^b*(i-1)+j},$$ where $j$ is an integer in $\{0,1, \ldots, 2^b-1\}$ with bit representation $\ind_i.$
% \end{definition}

% We can now formally describe our random planting matrix:

% \begin{definition}[Random Planting Matrix] \label{def:random-planting-matrix}
% The random planting matrix $M$ has rows indexed by $(\{-1,1\}^b)^n$ and columns indexed by $\{-1,1\}^m$. For any row index $\ind$ and column index $x$, $M(\ind,x) = f( s(\ind,x)).$
% \end{definition}

% We now explain what the random planting matrix is. For any $S \subseteq [m]$, such that $|S|= n$, we can construct an instance $\I_S$ of CSP(P) on $m$ variables by arbitrarily associating each of the $n$ variables in $\I^{*}$ with a distinct variable in $S$. Thus, as a function $\I_S$ will depend only on variables with indices in $S$ out of $[m]$.

% Any row index $\ind$ describes a set $S \subseteq [m]$ of size $n$: the set is constructed by thinking of $m$ as $n$ blocks of $2^b$ variables each and choosing one variable from each block. Calling this set $S(\ind)$, it is then easy to see that $M(\ind,x) = c-\I_{S_{\ind}}(x).$ In other words, each row of the matrix $M$ corresponds to an instance $\I$ of CSP(P) obtained by planting $\I^{*}$ over a subset of $n$ variables chosen from $[m]$.

% \subsection{Reduction to Lifted Matrices} The non-negative rank of the matrix $M$ is a lower bound on the size of any linear program that achieves a $(c,s)$-approximation for CSP(P). This is a consequence of the following fact, which follows from an application of Farkas' lemma (first shown by \cite{Yan91}, see also \cite{Pas12}, \cite{BFPS12}) that relates the non-negative rank of the certain matrices and the size of linear programs that achieve $(c,s)$-approximation for CSP(P).

% \begin{fact}[Non-negative Rank and LP Size]
% Let $\cQ$ be the collection of CSP(P) instances $\I$ such that $\opt(\I) = s > 0.$ For $c> s$, let $\cM_{=s}$ be the matrix with rows indexed by elements of $\cQ$ and columns by $\{-1,1\}^n$ such that $M_{=s}(\I,x) = c-\I(x)$. Then, there exists an LP relaxation of CSP(P) of size $R$ achieving a $(c,s)$ approximation if and only if $\nnr(M_{=s}) \leq R.$  \label{fact:nnrvslpsize}
% \end{fact}

% Combining the above fact with the observation that for every $\I_S$ obtained by planting $\I^{*}$ on the subset of variable $S \subseteq [m]$, $|S| = n$, the $\opt(\I_S) = \opt(\I^{*}) = s$ and thus $M$ is a sub-matrix of $M_{=s}.$

% \begin{corollary}
% Suppose there exists an LP relaxation for CSP(P) of size $R$ that achieves $(c,s)$-approximation. Then, $R \geq \Theta(\nnr(M)).$
% \end{corollary}

% The key technical lemma that reduces our job to lower bounding the non-negative rank of a lifted matrix is the following:

% \begin{lemma}
% Let $M$ be the random planting matrix constructed with positive integer parameters $b,n,c$ from the instance $\I^{*}$ of CSP(P). Then, $\nnr(M) \geq \nnr(M_f).$
% \end{lemma}
% \begin{proof}
% We will show that $M_f$ is a submatrix of $M.$ Specifically, let $q \in \on^{bn}$. We think of $q$ as $n$ blocks of $b$ bits each and write $q^1, q^2, \ldots, q^n$ to denote these $b$ blocks. For each choice of $q \in \on^{bn}$, we will associate a $x_q$ such that $M_f(\ind,q) = M(\ind,x_q),$ yielding our claim.

% We think of each $x \in \on^{2^bn}$ as $n$ blocks of $2^b$ bits each. Fix an arbitrary $q$ and let $x_q$ be the unique $x \in \on^{2^bn}$ that satisfies for each $i$, $\langle \ind_i, q \rangle = x^{i}$ where the inner product on the LHS here is the standard bilinear form on GF(2). Observe that such an $x$ exists and is unique to complete the proof.
% \end{proof}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%COMMENTED OUT COMMENTED OUT
% \fi


\section{Juntas, Rectangles, and Non-negative Rank of Lifted Matrices}

In this section, we will show our main \prettyref{thm:nnrlift} assuming \prettyref{thm:mainjunta}. Let $f:\on^n \to \rnng$ be as in the theorem with $\E[f] = 1$, and let the gadget $g:[q] \times [q] \to \on$ and $b$ be as in the theorem. We will show that if $\nnr(M_f)$ is small, then $\degp(f+\eta)$ is small, where $\eta = O(1/n)$. Concretely, given a small rank non-negative factorization of $M_f$, we use the factorization to get a small-degree conical junta approximating $f+\eta$. As described in the introduction, this is done in two modular steps: Lemmas \ref{lem:approx-conical}, and \ref{lem:approx-to-exact}.

Throughout this section we adopt the following assumptions:

%In this section, we reduce the task of proving a lower bound on the non-negative rank of a $f$ (i.e. Theorem \ref{th:nnrlift}) to showing the junta-approximation theorem which is the main technical contibution of the paper and the focus of the next section.

\begin{center}
  \fbox{\begin{minipage}{\textwidth}
  \paragraph{Important Parameters}
 \begin{itemize}
 	\item $f:\on^n \rightarrow \R_+$ with $\E[f] = 1$.
    \item The \emph{block-length} of the gadget $b = C \log_2 n$ for a sufficiently large constant $C$. (Recall that the gadget is the inner-product function).
\end{itemize}

  \end{minipage}}
\end{center}

%\pnote{Tried to write an overview (Commented out). Now don't like it so much.}
% \subsection{Proof Overview} \pnote{Writing a longish overview both to help me organize the proof and figure out what to stress and hopefully push most of it to the proof overview section in the intro later.}

% By our construction of $M_f$ from $f$ using the gadget $g$, for any $z \in \on^n$ and any $(x,y)$ such that $g^{\otimes n}(x,y) = z$, we must have:  $M_f(x,y) = f(z).$ In particular, let
% \begin{equation} A(z) = \E_{(x,y) \sim {g^{\otimes n}}^{-1}(z)}[ M_f(x,y)]. \label{eq:ffromaveraging}.
% \end{equation}
% Then, $f(z) = A(z)$ for every $z \in \on^n.$

% The idea of the proof is to show that if $M_f$ has low non-negative rank then, $A(z)$ is "simple". A priori, we could hope that ``simple'' really means having small non-negative degree. Then, we could start by assuming that $M_f$ has a low non-negative rank, say $R$ and combine the given lower bound on $\degp(f)$ with an upper bound on the $\degp(A)$ and obtain a contradiction using \eqref{eq:ffromaveraging}. However such a result is too strong and in fact false.

% We could relax our hope and try to show that low non-negative rank of $M_f$ implies that $A$ is ``close'' to some function with low non-negative degree. If we could argue that not only $\degp(f) > d$ but in fact, any small perturbation of $f$ cannot have non-negative degree $\leq d$, then we would still obtain a contradiction and be done. Thus, we start from the stronger assumption that $\degp(f+\eta) >  d$ for an appropriate non-negative $\eta.$

% How would we define closeness?  Chan et. al. \cite{CLRS13} developed a natural measure of closeness that we will also use in this paper. Consider the set of all $h:\on^n \rightarrow \R^{+}$ such that $\degp(h) \leq d.$ Then, this set is convex and thus, there must exist a linear operator on functions on $\on^n$, say $\cL$, such that $\cL(h) \geq 0$ for every $h$ such that $\degp(h) \leq d$ while $\cL(h') <0$ whenever $\deg(h') > d.$ To fix scales, we could fix $\cL(\1) = 1$ and for any function $h$, use $\cL(h)$ as a measure of how close $h$ is to being of non-negative degree at most $d$.

% Observe that under this measure, $f+\eta$ satisfies $\cL(f+\eta) < 0$ or $\cL(f) < -\eta.$ Now, if we could show that $\cL(A) > -\eta$ then we would obtain a contradiction and be done.

% How would we translate a non-negative rank upper bound on $M_f$ into a lower bound on $\cL(A)$? We start with the rank $1$ decomposition of $M_f$: there must be $R$ non-negative, rank 1 matrices $M_1, M_2, \ldots, M_R$ such that $$M_f  = \sum_{i = 1}^{R} \lambda_i M_i,$$ for some non-negative coefficients $\lambda_i$ chosen so that $\E[M_i] = 1$ for every $i.$ Rank 1 non-negative matrices  (especially when they are Boolean) are referred to as \emph{rectangles} in communication complexity.

% Just as for $M$, we could now define $A_i (z) = \E_{(x,y) \sim {g^{\otimes n}}^{-1}(z)}[ M_i(x,y)]$ for any $z \in \on^n$. Then, $A(z)  = \sum_{i = 1}^{R}  \lambda_i A_i(z).$ Thus, we could show that $\cL(A_i) > -\eta/(\sum \lambda_i)$, then we would be done.

% \textbf{Key Idea - Junta Approximation for Rectangles:} \pnote{Compare to CLRS here. Dropping this for now.}


% A natural way to show that $\cL(A_i)$ is lower bounded is to come up with an explicit approximator $h$ for $A_i$ that satisfies $\degp(h) \leq d$ and write $A_i = h + \err$ for some error. Observe that we only want to approximate $A_i$ by $h$ in the $\cL$-``norm''. Thus, while in standard distance measures $\err$ could be large, we are okay so long as $\cL(\err)$ is small.


% Observe that $M_i = pq^{\trsp}$ by virtue of being of non-negative rank $1$ for non-negative vectors $p,q \in \on^{bn}$. $\E[M_i] = 1$ forces $\E[p] = \E[q] = 1$ and thus, $p,q$ are \emph{densities} of probability distributions on $\on^n$. Further, $M_i(x,y)$ corresponds to the probability of the pair $(x,y)$ where $x$ and $y$ are chosen independently according to $p$ and $q$ respectively.

% It is not hard to show that a non-negative rank upper bound of $R$ on $M_f$ implies that WLOG, we can assume that $p$ and $q$ correspond to probability distributions with min-entropy at least $bn-t$ for $t = \log_2{(R)}.$ Our goal is thus obtain a lower bound on $\cL(A_i)$ where $M_i = pq^{\trsp}$ for $p,q$ densities of distributions with min-entropy at least $bn-t$ each.

% \pnote{Talk about extractor here:} How does the high min-entropy assumption on $p$, $q$ help? Here's where our choice of the gadget $g$ comes in. Observe that for any $z \in \on^n$, $A_i(z) = \E_{(x,y) \in {g^{\otimes n}}^{-1}(z)}[ p(x)q(y)].$ Equivalently, this is the probability under the product distribution $p \times q$ of a random pair $(x,y)$ satisfying ${g^{\otimes n}}^{-1}(x,y) = z.$ The Boolean inner product function is a strong \emph{randomness extractor}. That is, $g(x,y)$ for any


% We now want to use this flexibility to come up with a decomposition $h+\err$ for some $h$ satisfying $\degp(h) \leq d$ and $|\cL(\err)|$ is small. Our main technical contribution is to obtain such an approximation for $A_i$ obtained from arbitrary rectangles and is the focus of the following section.


% \pnote{ commented out for deletion:
% From here on, our proof can be broken into two broad steps. In the first step, our plan is to use the fact that $A$ is obtained by averaging over $\gtni(z)$ combined with a bound $\nnr(M_f)$ and obtain that $A$ must be ``close'' to having non-negative degree at most $d$.

% If we could ensure the stronger conclusion that $A$ has small non-negative degree from above, then we would be immediately done. However, such a conclusion cannot hold and to salvage the situation, we need to work with a notion of closeness that goes well with the kind of approximation we obtain above. It turns out that this notion of closeness, while being far from the standard norms, still has a nice interpretation and corresponds to the correlation with an appropriately chosen function $\cL$. To complete the proof, then, we will show that $\degp(f+\eta) > d$ yields an upper bound on $\cL(f)$ while our approximation for $A$ above yields a lower bound for $\cL(A)$ taken together yielding a contradiction when $R$ is too small.

% Next, we begin with the details of the two steps above. Bulk of the technical work goes into accomplishing the first step above leading to bounds on error of approximation of certain functions associated with non-negative rank 1 matrices by non-negative juntas. We only state the result in the next subsect - the proof of this theorem is the central technical contribution of this paper and is the focus of the next section.
% }

\subsection{Approximation by Approximate Conical Juntas}

Here we prove \prettyref{lem:approx-conical} which we restate for convenience.

\begin{lemma}[Non-negative rank to Approximate Conical Juntas]% \label{lem:approx-conical}
There exists a constant $\alpha_1 \geq 1$ such that the following holds. Let $f:\on^n \to \R_+$ with $\E[f] = 1$ and let $r = \nnr(M_f^b)$ for $b \geq \alpha_1 \log_2 n$. Then, $f$ is a $(2^{-b/2},2^{-bd/\alpha_1})$-approximate conical $d$-junta for all $d \geq \alpha_1 (\log r)/b$.
\end{lemma}
\ignore{
\begin{lemma}[Non-negative rank to Approximate Conical Juntas]
There exists a constant $\alpha_1 \geq 1$ such that the following holds. Let $f:\on^n \to \R_+$ with $\E[f] = 1$ and let $r = \nnr(M_f)$ with block-length $b \geq \alpha_1 \log_2 n$. Then, $f$ is a $(2^{-b/2},2^{-bd/\alpha_1})$-approximate conical $d$-junta for all $d \geq \alpha_1 (\log r)/b$.
\end{lemma}}

\begin{proof}
For the sake of brevity, let us set $G \seteq g^{\otimes n}$.  For every $z \in \on^n$, and $(x,y) \in G^{-1}(z)$, we have $M_f(x,y) = f(z)$. The high-level idea is as follows. From the definition of $M_f$, we have
 $$ f(z) =  \E_{(X,Y) \sim G^{-1}(z)}[ M_f(X,Y)].$$
% Then,  \begin{equation} A(z) = f(z) \end{equation} for every $z \in \on^n$.
Further, by definition of $\nnr(M_f)$, the matrix $M_f$ can be expressed as a sum of $\nnr(M_f)$ {\it non-negative rank-1 matrices}.  In turn, this yields a decomposition of $f$ into a sum of a family of non-negative functions. We then use Theorem \prettyref{thm:mainjunta} to approximate each of these functions by approximate conical juntas, thereby yielding the desired approximation for $f$.

Concretely, from the definition of non-negative rank, there exists a collection of densities on $\on^{bn}$, $\{u_i \mid 1 \leq i \leq R\}$ and $\{v_i \mid 1 \leq i \leq R\}$, and a set of non-negative constants $\lambda_1, \lambda_2, \ldots, \lambda_R$ such that $$M_f = \sum_{i = 1}^R \lambda_i u_i v_i^{\dagger}.$$
Observe that $$\sum_{i = 1}^R \lambda_i = \sum_{i = 1}^R \lambda_i = \sum_{i = 1}^R \lambda_i \E[ u_iv_i^{\dagger}]= \E[M_f] = 1.$$

Now, for any $z \in \on^n$,
\begin{align*}
f(z) &= \E_{(X,Y) \in G^{-1}(z)}[M_f(X,Y)]\\
&= \E_{(X,Y) \in G^{-1}(z)}\sbkets{\sum_{i=1}^R \lambda_i u_i(X) v_i(Y)}\\
&= \sum_{i=1}^R \lambda_i \cdot \E_{(X,Y) \in G^{-1}(z)}[u_i(X) v_i(Y)]\\
&= \sum_{i=1}^R \lambda_i \cdot Acc_{u_i,v_i}(z).
%&= \sum_{i=1}^R \lambda_i \cdot \E[\1_z(x,y) u_i(x) v_i(y)],
\end{align*}
(Recall the definition of $Acc$ from Equation \prettyref{eq:defacc}.)
\ignore{where we define $\1_z(x,y):[q]^n \times [q]^n \to \R_+$ by $\1_z(x,y) = (q^{2n}/|G^{-1}(z)|) \cdot \1(G(x,y) = z)$. Note that $\1_z$ is a density and in particular $\E[\1_z] = 1$. }
%\[ f(z) = \sum_{i = 1}^R \lambda_i \E[\1_z(x,y) u_i(x) v_i(y)] \mper\]

In analogy with communication complexity, we will refer to the rank $1$ matrices $u_i v_i^\dagger$ as {\it rectangles}. We will split the family of rectangles in to {\it large} and {\it small}.  To this end, fix $t = 4 \log_2{(R)}$.
%
A rectangle $u_i v_i^{\dagger}$ will be referred to as {\it large}, if the min-entropies of $u_i$ and $v_i$ are large.  More precisely, let
%\[Q \subseteq [R] = \{i \mid \| u_i \|_{\infty} \leq 2^{t/2} \text{ and } \| v_i \|_{\infty} \leq 2^{t/2} .\}\]
$$Q = \{i \in R\mid H_\infty(u_i) + H_\infty(v_i) \geq 2 (n-t) (\log q)\}.$$
%Clearly, by definition, $H_{\infty}(u_i) + H_{\infty}(v_i) \geq 2n-t$ for each $i \in Q.$
We can now write $f$ as a sum $f = J + \delta_1$ where,
\[J(z) = \sum_{i \in Q} \lambda_i Acc_{u_i,v_i}(z)\] and
\[ \delta_1(z) = \sum_{i \not \in Q} \lambda_i Acc_{u_i,v_i}(z) .\]

%\[J(z) = \sum_{i \in Q} \lambda_i \E[ \1_z(x,y) u_i(x) v_i(y)],\] and
%\[ \delta_1(z) = \sum_{i \not \in Q} \lambda_i \E[ \1_z(x,y) u_i(x) v_i(y))]) .\]

%By definition, for each $i \in Q$,  $H_{\infty}(u_i) + H_{\infty}(v_i) \geq 2n(\log_2 q) -t$; thus, for all $i \in Q$, by Theorem \prettyref{th:mainjunta}, $Acc_{u_i,v_i}$ is a $(\epsilon,\epsilon^d)$-approximate conical $d$-junta for all $d \geq \alpha_2 t/b$.
Now, for each $i \in Q$, by \prettyref{thm:mainjunta} applied to $u_i,v_i$, $Acc_{u_i,v_i}$ is a $(\epsilon,\epsilon^d)$-approximate conical $d$-junta for all $d \geq \alpha_2 t$. Therefore, $J$ is an $(\epsilon,\delta')$-approximate conical $d$-junta with $\delta' = \left(\sum_{i \in Q} \lambda_i \right) \cdot \epsilon^d \leq \epsilon^d$. %\PRnote{do we need to lose an $R$ here?  seems unnecessary since $\sum_i \lambda_i = 1$}.



\ignore{
In \prettyref{lem:mainjunta}, we will show that for any such {\it large} rectangle, the function
\[A_{u_i,v_i}(z) = \E[\1_z(x,y) u_i(x) v_i(y)] \mcom\]
is an $(\epsilon,\delta)$-approximate conical $d$-junta with $\epsilon = 2^{-0.5b}$ and $\delta = \epsilon^d$ for all $d \gg t/b$.}  %

%Applying Lemma \ref{lem:mainjunta} to $u_i,v_i$ for every $i \in Q$, we have:
%\begin{equation}
%A_{u_i,v_i}(z) = \sum_{j = 1}^{N } \lambda_{ij} C_{ij}(z) (1 + h_{ij}(z)) + \lambda_{i,err} \gamma_i,
%\end{equation}
%where, $\lambda_{i,j}, 2^{-t} \geq \lambda_{i,err} \geq 0$, $\sum_{j} \lambda_{i,j} + \lambda_{i,err} = 1$, $C_{ij}$s are $d$-conjunctions, $\gamma_i$ are densities and $h_{i,j}$ are $\epsilon$-decaying for $\epsilon = 2^{-0.5b}.$

Now we will bound the total additive error due to the small rectangles.  Observe that for any $i \not \in Q$, $\lambda_i \leq 2^{-t/2}$. This is because, $\lambda_i \E_{y}[ u_i(x) v_i(y)] = \lambda_i u_i(x) \leq \E_y[ M_f(x,y)] = \E[f] = 1$ and similarly, $\lambda_i v_i(y) \leq 1$ for any $y$. Further, recall that $Acc_{u,v}$ is a density for all densities $u,v$. Thus,
$$\E[\sum_{i \notin Q} \lambda_i A_{u_i,v_i}] \leq \sum_{i \notin Q} 2^{-t/2} \leq 2^{-t/2} R.$$
\ignore{
Now, $\E_{z} \E[ \1_z(x,y) u_i(x) v_i(y)] = \E_{x,y}[ u_i(x) v_i(y)] = 1.$ Thus, $\E[\delta_1] = \sum_{i \not \in Q} \lambda_i \leq 2^{-t/2} R.$ }

Therefore, $f = J+\delta_1$ is an $(\epsilon,\epsilon^d + 2^{-t/2}R)$-approximate conical $d$-junta for all $d \geq \alpha_2 t/b$. Choosing $t = 4 \log_2 R$ and $d = \max\{4\alpha_2 \log_2 R/b, 2\log_2 R/b\}$ proves the lemma.
%Thus, $J(z) = \sum_{i \in Q, j} \lambda_{ij} \cdot \lambda_{ij} C_{ij} (1+h_i)) + \sum_{i} \lambda_{i,err} \gamma_i$.
%
%Define $\delta(z) = \sum_{i} \lambda_{i,err} \gamma_i (z) + \delta_1(z).$ Then, $\E[ \delta] = \sum_{i,err} \lambda_{i,err} + \E[ \delta_1]$
%Similarly, $\sum_{i} \lambda_{i,err} \leq R 2^{-t} \leq 1/R.$  Thus, $\E[ \delta] \leq 2/R.$
\end{proof}




% \pnote{COMMENTED OUT, WILL DELETE:
% \subsection{$A$ is an Approximate Conical Junta}
% The goal of this section is to use Lemma \ref{lem:mainjunta} and arrive at an approximation for $A$ as a $\log{(R)}$-degree  conical junta.

% \begin{lemma}[Conical Junta Approximation for $A$]
% Let $R = \nnr(M_f)$. Then, there exist $J, \delta:\on^{m} \rightarrow \R^{+}$ satisfying $$A(z) = J(z) + \delta(z)$$ such that $d = \alpha_1\log_2{(R)}/b$ and $\epsilon = 2^{-\alpha_2b}$ for some constants $\alpha_1, \alpha_2$:
% \begin{enumerate}
% \item  there exist conical $d$-juntas $C_1, C_2, \ldots, C_N$, $\epsilon$-decaying functions $h_i$ and non-negative constants $\lambda_i$ such that $\sum_{i = 1}^R \lambda_i = 1$ and $$J(z) = \sum_{i} \lambda_i c_i (1 + h_i),$$

% \item $$\E[ \delta] \leq 2/R.$$
% \end{enumerate}
% \label{lem:simpleapprox}
% \end{lemma}


% \begin{proof}
% Since $\nnr(M_f) = R$, there exists a collection of densities on $\on^{bn}$, $\{u_i \mid 1 \leq i \leq R\}$ and $\{v_i \mid 1 \leq i \leq R\}$ and a set of non-negative constants $\lambda_1, \lambda_2, \ldots, \lambda_R$ such that $$M_f = \sum_{i = 1}^R \lambda_i u_i v_i^{\dagger}.$$ Observe that $$\sum_{i = 1}^R \lambda_i = \sum_{i = 1}^R \lambda_i = \sum_{i = 1}^R \lambda_i \E[ u_iv_i^{\dagger}]= \E[M_f] = 1.$$

% Fix $t = 4 \log_2{(R)}$. Let $Q \subseteq [R] = \{i \mid \| u_i \|_{\infty} \leq 2^{t/2} \text{ and } \| v_i \|_{\infty} \leq 2^{t/2} \}$. Then, $H_{\infty}(u_i) + H_{\infty}(v_i) \geq 2n-t$ for each $i \in Q.$ Observe that for any $i \not \in Q$, $\lambda_i \leq 2^{-t/2}$. This is because, $\lambda_i \E_{y}[ u_i(x) v_i(y)] = \lambda_i u_i(x) \leq \E_y[ M_f(x,y)] = \E[f] = 1$ and similarly, $\lambda_i v_i(y) \leq 1$ for any $y$.

% Let $$\delta_1(z) = \sum_{i \not \in Q} \lambda_i \E[ \1_z(x,y) u_i(x) v_i(y))])$$ and $$J(z) = \sum_{i \in Q} \lambda_i \E[ \1_z(x,y) u_i(x) v_i(y)].$$

% In this notation, thus, $$f(z) = \E[ \1_z(x,y) M_f(x,y)] = J(z) + \delta_1(z).$$

% From above, we know that for each $i \in Q$,  $H_{\infty}(u_i) + H_{\infty}(v_i) \geq 2n-t$.


% Applying Lemma \ref{lem:mainjunta} to $u_i,v_i$ for every $i \in Q$, we have:
% \begin{equation}
% A_{u_i,v_i}(z) = \sum_{j = 1}^{N } \lambda_{ij} C_{ij}(z) (1 + h_{ij}(z)) + \lambda_{i,err} \gamma_i,
% \end{equation}
% where, $\lambda_{i,j}, 2^{-t} \geq \lambda_{i,err} \geq 0$, $\sum_{j} \lambda_{i,j} + \lambda_{i,err} = 1$, $C_{ij}$s are $d$-conjunctions, $\gamma_i$ are densities and $h_{i,j}$ are $\epsilon$-decaying for $\epsilon = 2^{-0.5b}.$

% Thus, $J(z) = \sum_{i \in Q, j} \lambda_{ij} \cdot \lambda_{ij} C_{ij} (1+h_i)) + \sum_{i} \lambda_{i,err} \gamma_i$.

% Define $\delta(z) = \sum_{i} \lambda_{i,err} \gamma_i (z) + \delta_1(z).$ Then, $\E[ \delta] = \sum_{i,err} \lambda_{i,err} + \E[ \delta_1]$

% Now, $\E_{z} \E[ \1_z(x,y) u_i(x) v_i(y)] = \E_{x,y}[ u_i(x) v_i(y)] = 1.$ Thus, $\E[\delta_1] = \sum_{i \not \in Q} \lambda_i \leq 2^{-t/2} R \leq 1/R.$ Similarly, $\sum_{i} \lambda_{i,err} \leq R 2^{-t} \leq 1/R.$  Thus, $\E[ \delta] \leq 2/R.$
% \end{proof}
% }

\subsection{Approximate Conical Juntas to Conical Juntas}

\begin{center}
  \fbox{\begin{minipage}{\textwidth}
  \paragraph{Notation}
 \begin{itemize}
 	\item $\cC_{\leq D}$: cone of non-negative $D$-juntas on $\on^{n}.$
 	\item $\cL: \on^n \rightarrow \R$: separating function.
\end{itemize}
  \end{minipage}}
\end{center}


% \pnote{commented out for deletion:
% In the previous section, we showed that there's a certain conical junta approximation for $A$. In this section, we will develop tools required to show that $f$ cannot have an approximator of the form developed in the previous section if $\degp(f+\eta) > D = 2d.$ That is, the main goal of this section is the following lemma:

% \begin{lemma}
% Let $d,D$ be positive integer parameters satisfying $d <4D$ and for $\eta = 1/n$, let $\degp(f+\eta) > D.$  Then, there is a degree $D$ function $\cL$ such that for any non-negative $d$-junta $c$ satisfying $c(x) \leq 1$ for every $x$ and any $\epsilon$-decaying function $h$, for $\epsilon < \frac{1}{n^4},$ $\E[ \L c (1+h)] \geq - \epsilon^{3d} n^{4d}, $ while $\E[ \cL(f+\eta)] < 0.$
% \end{lemma}
% }

In this section we show \prettyref{lem:approx-to-exact} saying that if $f$ is a low-degree approximate conical junta, then $f+\eta$ is a low-degree conical junta for $\eta$ sufficiently small.%; the lemma essentially says that low-degree approximate conical juntas for sufficiently small error are in fact very close to being low-degree conical juntas.

%the class of conical juntas are \emph{robust} in a certain sense. Specifically, we will show that if $f$ is an $(\epsilon,\delta)$-approximate conical $d$-junta for a sufficiently small $\epsilon$ and $\delta$, then $f + \eta$ is a conical $O(d)$-junta for some small $\eta$.

\begin{lemma}
Let $f : \on^n \to \R^+$ with $E[f] = 1$ be a $(\epsilon,\delta)$-approximate conical $d$-junta for $\epsilon < 1/n^4$ and $\delta < 1/n^{8d}$. Then, \[ \degp(f+\frac{1}{n}) < 8d.\]
\end{lemma}

At a high-level the proof is as follows. Suppose for the sake of contradiction that $\degp(f+1/n) \geq 8d$. Then, there is a \emph{nice separating} functional $\L$ such that $\iprod{\L,f} \leq -1/n$, and $\iprod{\L,h} \geq 0$ for all $h \in \C_{< 8d}$. We then use further properties of the functional that the latter property implies $\iprod{\L,h} > -1/n$ for all $(\epsilon,\epsilon^d)$-approximate conical $d$-junta - leading to a contradiction.

We first develop the requisite technical machinery concerning conical juntas and separating functionals.


%\PRnote{Include some overview.}
% \subsection{Overview}

% How would we define the measure of closeness?  Chan et. al. \cite{CLRS13} developed a natural measure of closeness that we will also use in this paper. The next subsection describes this measure and also proves some elementary facts about it that we will need in the proof.

% Consider the set of all $h:\on^n \rightarrow \R^{+}$ such that $\degp(h) \leq d.$ Then, this set is convex and thus, there must exist a linear operator on functions on $\on^n$, say $\cL$, such that $\cL(h) \geq 0$ for every $h$ such that $\degp(h) \leq d$ while $\cL(h') <0$ whenever $\deg(h') > d.$ To fix scales, we could fix $\cL(\1) = 1$ and for any function $h$, use $\cL(h)$ as a measure of how close $h$ is to being of non-negative degree at most $d$. Formally, we have:

\begin{lemma} \label{lem:sadual}
Suppose $D < \degp(f+\eta).$ There exists a degree $D$ function $\L:\on^{n} \rightarrow \R$ such that:
\begin{enumerate}
\item $\E[ \L ] = \E[ \L \cdot 1] = 1$.
\item $\E[ \L f] < -\eta$.
\item $\E[ \L h] \geq 0$ for every conical $D$-junta $h$ on $\on^n.$
\item $|\hat{\L}(S)| \leq 1$ for every $|S| \leq D$.
\item $\norm{\L}_{\infty} \leq n^{D}$
\end{enumerate}
\end{lemma}
\begin{proof}
Observe that the set of conical $\leq D$-juntas denoted by $\cC_{\leq D}$ is convex. On the other hand from the hypothesis, we have that $f +\eta \not \in \cC$. Thus,
there exists a function $\L:\on^n \rightarrow \R$ such that $\langle \L, h \rangle \geq 0$ for every $h \in \cC_{\leq d}$ but $\langle \L , (f+\eta) \rangle < 0$.  Moreover, since $\cC_{\leq D}$ is contained in the linear subspace of degree $D$ polynomials, without loss of generality, we can assume that $\L$ is also a degree $D$ polynomial.

The first three properties are simple to verify. Since the constant function $\1 \in \cC_{\leq D}$, we can assume (by rescaling, if needed) that $\langle \L , 1 \rangle = 1$ giving us the first property. Further, since $\langle \L , f \rangle = \L \cdot (f+\eta) - \langle \L , \eta \rangle \leq -\eta$ giving us the second property. The third property follows from our definition of $\L$.

%For every subset $J \subset[n]$ of size $\leq D$ and a partial assignment $\alpha \in \{-1,1\}^J$, the indicator function $\1[x_{J} = \alpha]$ is a non-negative junta and therefore satisfies $\langle \L ,\1[x_{J} = \alpha] \rangle \geq 0$ by our choice of $\L$.  If $h$ is any non-negative $D$ junta depending on variables with the indices contained in $J$, then, $h$ is a non-negative linear combination of $\1[ x_{J} = \alpha]$ and thus by linearity of inner product $\langle \L, h \rangle \geq 0$ giving us the third property.


We next bound the Fourier coefficients of $\L$. First observe that for any $S \subseteq [n]$, $|S| \leq D$, $\1+\chi_S$ is a non-negative $D$-junta. Therefore, $\iprod{\L,1+\chi_S} \geq 0$ so that $\iprod{\L,\chi_S} \geq -\iprod{\L,1} = -1$. Similarly, $\iprod{\L,1-\chi_S} \geq 0$ so that $\iprod{\L,\chi_S} \leq 1$. Thus, $|\hat{\L}(S)| = |\iprod{L,\chi_S}| \leq 1$. 
\ignore{\begin{align*}
\left|\hat{L}(S) \right| = \left| \langle \L , \chi_{S}(x) \rangle \right| = \left|{\sum_{\alpha \in \{-1,1\}^S} \langle \L , \chi_{S}(\alpha) \cdot
  \1[x_{S } = \alpha]} \rangle \right| \leq \sum_{\alpha \in \{-1,1\}^S} \langle \L , \1[x_{S} = \alpha] \rangle = 1
  \end{align*}}

%The inequality above uses the fact that for any $\alpha \in \on^{S}$, from part three proven above, $\langle \L, \1[x_{S }  = \alpha] \rangle  \geq 0.$ The last equality follows from the observation that for any $S \subseteq [bn]$, $\langle \L, \sum_{\alpha \in \on^{S}} \1[x_{S} = \alpha] \rangle = \langle \L, \1 \rangle = 1.$  

The final property follows as $\norm{L}_{\infty} = \norm{\sum_{S, |S| \leq D} \hat{\L}(S) \chi_S(x)} \leq \sum_{|S| \leq D} \| \hat{\L}(S) \| < n^{D}$.
\end{proof}

The following technical property of $\L$ constructed in Lemma \ref{lem:sadual} will be required in our proof.

\begin{lemma}
Let $\L:\on^n \to \R$ be the separating function of degree $D$ given by Lemma \ref{lem:sadual}.  Let $h:\on^n \to \rnng$ be a  non-negative junta that depends only on variables $T \subseteq [n]$ and let $S$ be any subset of $[n]$ such that and $|S|+ |T| \leq D$. Then, $$\E[ \L h \chi_S] \leq \E[ \L h].$$ \label{lem:conditioning}
\end{lemma}

\begin{proof}
Note that $h(1-\chi_S)$ is a non-negative $D$-junta. Therefore, $\iprod{\L,h(1-\chi_S)} \geq 0$; the claim follows.
\ignore{
For $\1_{\chi_S(x) = 1}$ and $\1_{\chi_S(x) = -1}$, the $0$-$1$ indicators of the sets $\{ x \mid  \chi_S(x) = 1\}$ and $\{ x \mid \chi_S(x) = -1\}$ respectively, we have:
\begin{equation} \E[ \L c \chi_S]  = \E[ \L c \1_{\chi_S(x) = 1}] - \E[ \L c \1_{\chi_S(x) = -1}] \label{eq:temp1}
 \end{equation}
Now, $c \cdot \1_{\chi_S(x) = -1}$ is a conical $D$-junta from the assumption in the statement. Thus, $\E[ \L c \1_{\chi_S(x) = -1}] \geq 0$. Thus, \eqref{eq:temp1} yields:
$$\E[ \L c \chi_S]  \leq \E[ \L c \1_{\chi_S(x) = 1}] + \E[ \L c \1_{\chi_S(x) = -1}] = \E[ \L c].$$}
\end{proof}

We are now ready to prove Lemma \ref{lem:main-estimate} which can be seen as a robust version of the property that $\E[\cL h] \geq 0$ for every  non-negative $D$-junta $h$.

\begin{lemma} \label{lem:main-estimate}
Let $\L$ be a separating function of degree $D=4d$ as in Lemma \ref{lem:sadual}. Then, for any non-negative $d$-junta $c$ with $\|c\|_\infty \leq 1$, and any $(1/n^4)$-decaying function $h$, $\E[ \L c (1+h)] \geq -n^{-8d} $.
\end{lemma}

\begin{proof}
Write $h = h_{low} + h_{high}$ where $h_{low} = \sum_{|S| \leq D-d} \hat{h}(S) \chi_S,$ and $h_{high} = \sum_{|S| > D-d} \hat{h}(S) \chi_S.$

We have: $$\E[ \L c (1 + h)]  = \E[\L c (1 + h_{low})] + \E[ \L c h_{high}].$$
%Observe that since $|\hat{L}(S)| \leq 1$, $|\L(x)|\leq n^{D}$. 
Let $\epsilon = 1/n^4$. Now, $\L c$ is of degree at most $(D+d)$ and $\|\L c\|_\infty \leq n^D$. Further, for any $x$,
\begin{align*}
|h_{high}(x)| &= |\sum_{S: |S| \geq D-d} \hat{h}(S) \chi_S(x)| \leq \sum_{S: |S| \geq D-d} \epsilon^{|S|}\\
&\leq \sum_{\ell=D-d}^n \epsilon^\ell \cdot n^\ell\\
&\leq 2(\epsilon n)^{D-d},
\end{align*}
where the last inequality follows as $\epsilon n = 1/n^3 < 1/2$. Therefore, $\|h_{high}\|_\infty \leq 2 (\epsilon n)^{D-d}$ and 

%Noting that $h$ is $\epsilon$-decaying, $c$ is bounded above by $1$ and that $h_{high}$ is a linear combination of parities of degree at least $D-d$, we have:
\begin{equation}
|\E[ \L c h_{high}]| \leq \|\L c\|_\infty \cdot \|h_{high}\|_\infty \leq 2 n^{2D-d} \cdot \epsilon^{D-d}. \label{eq:part1}
\end{equation}

Next, note that $h_{low}$ is a linear combination of parities of degree at most $d$ and that $c$ is a function of degree at most $d$. Thus, by \prettyref{lem:conditioning}, we have,
\begin{align*}
|\E[ \L c h_{low}]| &\leq \sum_{|S| \leq D-d} |\hat{h}(S)| | \E[ \L c \chi_S]|\\
&\leq \sum_{|S| \leq D-d} |\hat{h}(S)| \E[ \L c].
\end{align*}

Since by definition $\E[h] = 0$, we have:
\begin{equation}
\E[ \L c (1 + h_{low})] \geq \E[ \L c ] (1 - \sum_{1 \leq |S| \leq D-d} \epsilon^{|S|}) \geq  \E[\cL c] (1- 2D n \epsilon). \label{eq:part2}
\end{equation}
Using that $\epsilon < 1/n^{4}$ and $D < n$, we have $E[ \L c (1 + h_{low})] \geq 0$. Using \eqref{eq:part1} and \eqref{eq:part2}, $$\E[\L c (1+h)] \geq - 2 \epsilon^{3d}n^{7d} \geq - n^{-8d}.$$
\end{proof}

Finally, we can complete the proof of \prettyref{lem:approx-to-exact}.
\begin{proof}[Proof of \prettyref{lem:approx-to-exact}]
Fix $\eta = \frac{1}{n}$.  For the sake of contradiction, assume that $\degp(f+\eta) \geq 8d$.  Consider the functional $\cL$ given by \prettyref{lem:sadual} with $D = 4d$.

Since $f$ is an $(\epsilon,\delta)$-approximate $d$-junta, we have
\[ f(z) = \sum_{i} \lambda_i c_i(z) (1 + h_i(z)) + \gamma(z) \]
where the functions $h_i$ are $\epsilon$-decaying and the function $\gamma$ satisfies $\E[|\gamma|] \leq \delta$.
Now, apply the linear functional $\cL$ to both sides of the above equation.  On one side, we get \[\E[ \cL \cdot f] \leq -\eta \mper \]
On the other side, we get
\begin{align*}
\sum_{i} \lambda_i \E[ \cL c_i (1+ h_i)] + \E[\cL \gamma]
& \geq - \left(\sum_i \lambda_i \right)  \cdot \frac{1}{n^{8d}} - \norm{\cL}_{\infty} \E[|\gamma|] \\
& \geq -\frac{1}{n^{8d}} - n^{4d} n^{-8d}  > -\eta \mcom
\end{align*}
%\PRnote{need to add a little more detail to above calculation}
yielding a contradiction.
\end{proof}


%\begin{proof}[Proof of Lemma \ref{lem:main-estimate}]
%We use the separating function $\cL$ constructed in Lemma \ref{lem:sadual}. The second property is then a direct consequence of Lemma \ref{lem:sadual}.
%\end{proof}

% \pnote{
% \subsection{Putting Things Together}
% We can now complete the proof of Theorem \ref{thm:nnrliftrestated}.

% \begin{proof}[Proof of Theorem \ref{thm:nnrliftrestated}]
% Recall: $R = \nnr(M_f)$, $A$, the acceptance function of $M_f$ and $\degp(f+\eta) > D.$ Suppose $R > n^{8d}.$
% Using Lemma \ref{lem:simpleapprox} we write: $A(z) = J(z) + \delta(z).$ Using Lemma \ref{lem:main-estimate}, we have (using that $A = f$)
% \begin{align*}
% \E[ \L (f +\eta)]  &= \E[\cL A] + \eta \\
% &= \E[ \L J] + \E[ \L \delta] + \eta \\
% &= \sum_{i} \lambda_i \E[ \L c_i (1+h_i)] + \E[ \L \delta] + \eta.
% \end{align*}
% Using non-negativity of $\delta$, we have:
% \begin{align*}
% &\geq (\sum_{i} \lambda_i) (- \epsilon^{D-d} m^{2D}) - \|\L\|_{\infty} \E[ \delta] +\eta \\
% &\geq -  2^{-1.5 bd} n^{4d} - 2n^{4d} /R + \eta.
% \end{align*}

% Choosing a large enough $b = \Theta(\log_{2}(n))$ for any $\eta > 1/n$, we thus have that $\E[ \cL( f+ \eta)] > 0.$

% On the other hand, from Lemma \ref{lem:sadual}, we know that $\E[\cL(f+\eta)] < -\eta + \eta = 0$ obtaining a contradiction. This completes the proof.
% \end{proof}
% }

\section{The Junta Approximation Theorem}
Here we prove \prettyref{thm:mainjunta} assuming \prettyref{thm:maindecomp}. In addition to the latter decomposition, the proof relies on certain \emph{extractor} properties of the inner-product function. Concretely, we need the following statement about the distribution of $G(X,Y)$ for block-wise dense random variables $X,Y$ that is implicit in \cite{GLMWZ15}.

\begin{lemma}\label{lem:bd-epsilon-decay}
Fix $q = 2^b$ for $b > 7$ and identify $[q]$ with $\on^b$.  Let $\iproduct : \zo^b \times \zo^b \to \on$ be the Boolean inner product function.

Suppose $X$ and $Y$ are independent, blockwise dense random variables on $[q]^{n}$. Let $\nu$ be the density of the random variable $\iproduct^{\otimes n} (X,Y)$ on $\on^n$. Then, $\nu = 1 + h$ for an an $\epsilon$-decaying function $h$ where $\epsilon =  2^{-0.5b}.$ \label{lem:bd-epsilon-decay}
\end{lemma}

The lemma is an easy consequence of the fact that the inner-product function is a \emph{two-source extractor} for sufficiently high-entropies:
%We will need the following fact in the proof. Recall that $g$ is the $b$ bit Boolean inner product function with outputs in $\on$.

\begin{fact}[Chor-Goldreich \cite{CG88}]\label{fact:ipextractor}
Suppose $X, Y $ are independent random variables over $\on^{\ell}$ for $\ell > 7$ with min-entropy $H_{\infty}(X),H_{\infty}(Y) \geq 0.8 \ell$. Then, %for the boolean inner product function $\iproduct$,
%\[|\Pr[ \iproduct(X,Y) = +1 ]-\half|  \leq 2^{-0.6 \ell} \mcom\]
%or equivalently,
\[|\E[\iproduct(X,Y)]| \leq 2^{-0.6 \ell + 1} \mper \]
\label{fact:Chor-Goldreich}
\end{fact}

% \begin{fact}[Chor-Goldreich \cite{CG88}]
% Suppose $X, Y $ are independent, blockwise dense random random variables over $\on^{bn}$ for $b > 7$. Then, for any $I \subseteq [n]$, $|\Pr[ \Pi_{i \in I} g(X_{\{i\}},Y_{\{i\}}) = +1 ] - 1/2| \leq 2^{-0.8b|I|}.$  \label{fact:Chor-Goldreich}
% \end{fact}
\begin{proof}[Proof of Lemma \ref{lem:bd-epsilon-decay}]
By Fact \ref{fact:Chor-Goldreich}, for any $S \subseteq [n]$ we have
\[ \hat{\nu}(S) = \E[ \nu(z) \chi_S(z)] = \E_{z \sim \nu}[ \chi_S(z)] = \E[\Pi_{i \in I} g(X_{\{i\}},Y_{\{i\}})] = \E[\iproduct(X_{S},Y_{S})].\]

Thus, $|\hat{\nu}(S)| \leq 2^{-0.6b|S|+1} < 2^{-0.5b}$.

Let $h(z) = \sum_{|S| \geq 1} \hat{\nu}(S) \chi_S(z).$ Then, $\nu = 1 + h$ and by the above estimate, $h$ is $\epsilon$-decaying for $\epsilon = 2^{-0.5b}.$
\end{proof}

Lemma \ref{lem:bd-epsilon-decay} showed that if $X,Y$ are $\bd$ random variables, then the density of $\iproduct^{\otimes n}(X,Y)$ is an $\epsilon$-decaying perturbation of the uniform density. In the following, we show a refinement of Lemma \ref{lem:bd-epsilon-decay} when $X,Y$ are aligned $d$-$\cbd$ random variables - specifically, that $g^{\otimes n}(X,Y)$ is a an $\epsilon$-decaying perturbation of a non-negative $d$-junta.

\begin{lemma}
Let $X,Y$ be aligned $d$-$\cbd$ random variables over $(\zo^{b})^n$ for $b > 7$ with the aligned blocks $I \subseteq [n]$ and $X_I = \alpha, Y_I = \beta$. Let $\nu$ be the density of $z = \iproduct^{\otimes n}(X,Y).$ Then, for $\epsilon  = 2^{-0.5b}$, there exists an $\epsilon$-decaying function $h$ such that
%
\[\nu = 2^{|I|} \cdot \1[z_I = \iproduct^{\otimes |I|}(\alpha, \beta)] \cdot (1+h).\] \label{lem:junta-approx-for-CBD}
In particular, if $u,v$ are aligned $d$-$\cbd$ densities over $(\on^b)^n$, then $Acc_{u,v}$ is a $(2^{-.5b},0)$-approximate conical $d$-junta.
\end{lemma}
%\PRnote{For events and indicator of events, I like $\1[E]$ over $\1(E)$}

%\pnote{use a standard symbol for the gadget g}

\PRnote{need a consistent notation for gadget $g$,and its special case, $\iproduct$.  I have chosen one here, hopefully we can find something better}
\begin{proof}
Let $Z = \iproduct^{\otimes n}(X,Y)$. Then, $Z_I = \iproduct^{\otimes I}(\alpha,\beta$ and $Z_{\bar{I}} = \iproduct^{\otimes |\bar{I}|}(X_{\bar{I}}, Y_{\bar{I}})$. %Since $X_I = \alpha$ and $Y_I = \beta$ are fixed, we have that $Z_I = \iproduct^{\otimes |I|}(\alpha, \beta).$ 
In particular, the density of $Z$ can be written as $\nu_I \cdot \nu_{\bar{I}}$ where $\nu_I$ is the density of $Z_I$ and $\nu_{\bar{I}}$ the density of $Z_{\bar{I}}$.

Now, by definition, $X_{\bar{I}}, Y_{\bar{I}}$ are $d$-$\cbd$ random variables. Thus, by \prettyref{lem:bd-epsilon-decay}, the density $\nu_{\bar{I}}$ of $Z_{\bar{I}}$ can be written as $1+h$ for a $2^{-0.5b}$-decaying function. This completes the proof of the first part of the statement. The next part follows from the definition of $Acc_{u,v}$.
\end{proof}

We are now ready to prove \prettyref{thm:mainjunta} which we restate for convenience.

\begin{theorem}[Junta Approximation]%\label{thm:mainjunta}
There exists a constant $\alpha_2 \geq 1$ such that the following holds. Let $u,v$ be densities over $[q]^n$ with $q =2^b$ such that $H_{\infty}(u)+ H_{\infty}(v) \geq 2b(n-t)$. Then, for all $b \geq \alpha_2 \log n$ and $d \geq \alpha_2 t$, $Acc_{u,v} \on^n \to \rnng$ is a $(2^{-0.5b},(2^{-0.5b})^d)$-approximate conical $d$-junta.

%and $\epsilon = 2^{-0.5b}$, $Acc_{u,v}:\on^n \to \R_+$ is a $(\epsilon,\epsilon^d)$-approximate conical $d$-junta.
\ignore{There exist $d$-conjunctions $C_1, C_2, \ldots, C_N:\on^n \to \R_+$, $\epsilon$-decaying functions $h_1,\ldots,h_N:\on^n \to \R$, a density $\gamma:\on^n \to \R_+$, and non-negative weights $\lambda_1,\ldots,\lambda_N, \lambda_{err} \geq 0$ such that
$$A_{p,q}(z) = \sum_{i=1}^N \lambda_i C_i(z) (1 + h_i(z)) + \lambda_{err} \gamma, $$
where $\sum_{i=1}^N \lambda_i + \lambda_{err} = 1$, and $|\lambda_{err}| \leq \epsilon^d$.}
\end{theorem}
\ignore{
\begin{theorem}
Let $u,v$ be densities over $\on^{bn}$ such that $H_{\infty}(u)+ H_{\infty}(v) \geq 2bn-t.$ Then, there exists a constant $\alpha_2 > 0$ such that for all $d \geq \alpha_2 t/b$ and $\epsilon = 2^{-0.5b}$, $Acc_{u,v}:\on^n \to \R_+$ is a $(\epsilon,\epsilon^d)$-approximate conical $d$-junta.
\end{theorem}}
\begin{proof}
We apply \prettyref{thm:maindecomp} to $u,v$ to write 
$$u \otimes v = \sum_{i =1}^N \lambda_i u_i \otimes v_i + \lambda_{error} \gamma_{error},$$
as guaranteed by the theorem. Then,
$$Acc_{u,v} = \sum_{i=1}^N \lambda_i Acc_{u_i,v_i} + \lambda_{error} \gamma(z),$$
where $\gamma$ denotes the distribution of $G(X,Y)$ for $(X,Y) \sim D_{error}$. Now, as $u_i,v_i$ are aligned $d$-\cbd densities, by \prettyref{lem:junta-approx-for-CBD} each $Acc_{u_i,v_i}$ is a $(2^{-.5b},0)$-approximate conical $d$-junta. Hence, $Acc_{u,v}$ is a $(2^{-.5b},\lambda_{err})$-approximate conical $d$-junta. The claim now follows from the bound on $\lambda_{err}$.
\ignore{
Let $X,Y$ be sampled according to the densities $u,v$ respectively. Then, we can apply \prettyref{thm:maindecomp} to $X \times Y$ (with $q = 2^b$ and $[q]$ identified with $\zo^b$) as they are independent and satisfy $H_\infty(X) + H_\infty(Y) \geq 2bn - t$. Let $X_i,Y_i,\lambda_i$ for $1 \leq i \leq N$, $\lambda_{err}, E$ be distributions as showed to exist in \prettyref{thm:maindecomp} for $d \gg t/b$ with $\lambda_{err} \leq 2^{-\Omega(bd)}$.
 Now, as we are writing the density of $X \times Y$ as a convex combination of $X_i \times Y_i$ and $E$, for all $z \in \on^n$,
$$\pr[G(X,Y) = z] = \sum_{i=1}^N \lambda_i \pr[G(X_i,Y_i) = z] + \lambda_{err} \pr_{(X',Y') \sim E}[G(X',Y') = z].$$
Therefore, if we let $u_i,v_i$ be the densities of $X_i,Y_i$ respectively for $1 \leq i \leq N$, then
$$Acc_{u,v}(z) = \sum_{i=1}^N \lambda_i Acc_{u_i,v_i}(z) + \lambda_err \gamma(z),$$
where $\gamma$ denotes the density of the distribution $G(X',Y')$ for $(X',Y') \sim E$. Now, \prettyref{lem:junta-approx-for-CBD}, each $Acc_{u_i,v_i}$ is a $(2^{-.5b},0)$-approximate conical $d$-junta. Hence, $Acc_{u,v}$ is a $(2^{-.5b},\lambda_{err})$-approximate conical $d$-junta. The claim now follows from the bound on $\lambda_{err}$.}

\ignore{
Recall that $A_{u,v}(z)  = \E[ \1_z(x,y) u(x)v(y)]$ where $z$ is the $2^n$ scaled $0$-$1$ indicator of $\{(x,y) \mid \iproduct^{\otimes n}(x,y) = z\}.$  Apply Lemma \ref{lem:maindecomp} to $u$ and $v$. Let $X_i, Y_i, \lambda_i, \nu_i$ for $1 \leq i \leq N$ and $\lambda_err,E$ be the output parameters of the decomposition of $pq.$

Then, $A_{u,v}(z) = \sum_{i = 1}^N \lambda_i \E[ \1_z(x,y) \nu_i(x,y)] + \lambda_{err} \E_{(x,y) \sim E}[ \1_z(x,y) E(x,y)].$ Let $\delta$ be the density induced on $\on^{n}$ by $E$,i.e., $\delta(z) = \E[ \1_z(x,y) E(x,y)].$

Observe that $\E[\1_z(x,y) \nu_i(x,y)]$ is just the density of $\iproduct^{\otimes n }(X_i,Y_i)$ and since $(X_i, Y_i)$ are aligned $d$-CBD, using Lemma  \ref{lem:junta-approx-for-CBD} we obtain for each $1 \leq i \leq N$,  non-negative $d$-conjunctions $J_i$, coefficients $C_i$ and $\epsilon$-decaying functions $h_i$ for $\epsilon = 2^{-0.5b}$ such that $\E[ \1_z(x,y) \nu_i(x,y)] = C_i J_i(z) (1+h_i(z)).$

This completes the proof. }
\end{proof}



\ignore{Consider the rank $1$ matrix $pq^{\trsp}$ where $p,q$ are non-negative vectors indexed by $\on^{m},$ satisfying $\E[p] = \E[q] =1.$ For any $z$, let $${g^{\otimes n}}^{-1}(z) = \{(x,y) \in \on^{m} \times \on^{m} \mid g^{\otimes n}(x,y) = z\}$$ and let $\1_z:\on^{m} \times \on^{m}$ be the mean $1$ indicator of $\gtn(x,y) = z$:
\begin{equation} \label{eq:mean1indicator}
\1_z(x,y) = \begin{cases} 2^n & \text{ if } \gtn(x,y) = z\\
             0 & \text{ otherwise. }
             \end{cases}
\end{equation}

Let $A_{p,q} = \E[ \1_z(x,y)p(x)q(y)]$ be the appropriately scaled probability of $(x,y) $



Next, for any $z \in \on^n$, we define $A_{p,q}(z)$ which is the probability under the product distribution defined by $p \times q$ on $\on^{bn} \times \on^{bn}$ of $(x,y)$ satisfying $\gtn(x,y) = z.$

\begin{definition}
Let $Q$ be a non-negative matrix with rows and columsn indexed by $\on^{bn}$ such that $\E[Q] = 1.$ Let $A_Q: \on^{n} \rightarrow [0,1]$ be defined by:

$$A_Q(z) = \E[ \1_z(x,y) p(x) q(y)],$$ where $\1_z$ is the mean $1$ indicator of $\{(x,y) \mid \gtn(x,y) = z\}$ defined in \eqref{eq:mean1indicator}. When $Q = pq^{\transposed}$ for densities $p,q \in \on^{bn}$, we write $A_{p,q}$ for $A_Q.$
\end{definition}

Our junta approximation theorem says that for densities $p,q$ with min-entropy at least $bn-t$, $A_{p,q}$ is essentially a conical junta of degree $O(t/b)$. %can be expressed as a perturbation of a non-negative junta of degree $d \approx t/b$. \pnote{say something meaningful about the multiplicative error and why it shows up and is important.}

\begin{theorem}[Junta Approximation]\label{th:mainjunta}
Let $p,q$ be densities over $\on^{bn}$ such that $H_{\infty}(p)+ H_{\infty}(q) \geq 2bn-t.$ Then, there exists a constant $\alpha_2 > 0$ such that for all $d \geq \alpha_2 t/b$ and $\epsilon = 2^{-0.5b}$, $Acc_{p,q}:\on^n \to \R_+$ is a $(\epsilon,\epsilon^d)$-approximate $d$-conical junta.
\ignore{There exist $d$-conjunctions $C_1, C_2, \ldots, C_N:\on^n \to \R_+$, $\epsilon$-decaying functions $h_1,\ldots,h_N:\on^n \to \R$, a density $\gamma:\on^n \to \R_+$, and non-negative weights $\lambda_1,\ldots,\lambda_N, \lambda_{err} \geq 0$ such that
$$A_{p,q}(z) = \sum_{i=1}^N \lambda_i C_i(z) (1 + h_i(z)) + \lambda_{err} \gamma, $$
where $\sum_{i=1}^N \lambda_i + \lambda_{err} = 1$, and $|\lambda_{err}| \leq \epsilon^d$.}
\end{theorem}

The theorem follows easily from our main decomposition result for product distributions, \prettyref{lem:maindecomp}, and properties of the inner-product function viewed as an \emph{extractor}. }

\ignore{
The goal of this section is to prove the junta approximation Lemma - Lemma \ref{lem:mainjunta}:
% \begin{lemma}[Junta Approximation, Lemma \ref{lem:mainjunta} restated]
% Let $p,q$ be densities over $\on^{bn}$ such that $H_{\infty}(p)+ H_{\infty}(q) \geq 2n-t.$ Then, there exist constants $\alpha_1, \alpha_2 > 0$ such that for $d = \alpha_1 t/b$ and $\epsilon = 2^{-\alpha_2 b}$, there exist sets $I_1,\ldots, I_N \subseteq [m]$ of size at most $d$, partial assignments $\gamma_i \in \on^{I_i}$, non-negative weights $\lambda_1,\ldots,\lambda_N \geq 0$, and $\epsilon$-decaying functions $h_1,\ldots,h_N$ such that
% $$A_{p,q}(z) = \sum_{i=1}^N \lambda_i \mathsf{1}(z_{I_i} = \gamma_i) \cdot (1 + h_i(z)) \pm \epsilon^d.$$
% \label{lem:mainjunta-restated-weaker}
% \end{lemma}

\pnote{What is proven in this section right now is the following weaker form that is enough for our purposes:}

\begin{lemma}[Junta Approximation, Theorem \ref{lem:mainjunta} restated]
Let $p,q$ be densities over $\on^{bn}$ such that $H_{\infty}(p)+ H_{\infty}(q) \geq 2bn-t.$ Then, there exist constants $\alpha_1, \alpha_2 > 0$ such that for $d = \alpha_1 t/b$ and $\epsilon = 2^{-\alpha_2 b}$, $d$-conjunctions $C_1, C_2, \ldots, C_N$, non-negative weights $\lambda_1,\ldots,\lambda_N, \lambda_{err} \geq 0$ such that $\sum_{i = 1}^N \lambda_i + \lambda_{err} = 1$, $\epsilon$-decaying functions $h_1,\ldots,h_N$ and a density $\delta$ on $\on^n$ such that
$$A_{p,q}(z) = \sum_{i=1}^N \lambda_i C_i(z) (1 + h_i(z)) + \lambda_{err} \delta, $$ for $\lambda_{err} \leq \epsilon^d.$ \label{lem:mainjunta-restated}
\end{lemma}}



\section{Decomposition of High Min-Entropy Distributions}
In this section we prove \prettyref{thm:maindecomp}. In fact, we show a generalization of the theorem where the error is small under a more general class of distributions; this generalization is not needed for the rest of the results but is no more difficult to prove and is needed to recover the results of \cite{GoosLMWZ15} in our framework.

We will use the following notation:
\begin{itemize}
	\item We use distributions, densities and random variables interchangeably with the meaning being clear from the context.
	\item For $\mu$ a density on some domain $\cal{D}$ and $S \subseteq \cal{D}$, we write $\mu_{|S}$ for the density $\mu$ conditioned on $S$. We also define $\mu(S) = \pr_{X \sim \mu}[X \in S]$.
	\item For a random variable $X$ on $[q]^n$ and $I \subseteq [n]$, we write $X_I$ to denote $X$ projected to the coordinates in $I$. For a density $\mu$ on $[q]^n \times [q]^n$ and $I \subseteq [n]$, we write $\mu_I$ to denote the density on $[q]^{|I|} \times [q]^{|I|}$ obtained by projecting $\mu$ to the cooridnates in $I$. 
	\item For brevity, we say a density $\mu$ on $[q]^n \times [q]^n$ is an aligned $d$-\cbd if its two marginals along $[q]^n$ are aligned $d$-\cbd densities. 
 %   \item For a random variable $Y$ on $[q]^n$, $I \subseteq [n]$, and $\alpha \in [q]^I$, we write $(Y \mid Y_I = \alpha)$ for the random variable $Y$ conditioned on the event $Y_I = \alpha.$
    %\item For $\mu$, a density on $[q]^n \times [q]^n$, and any subset $S \subseteq [q]^n \times [q]^n$, we write $\mu(S)$ for $\Pr_{(x,y) \sim \mu}[ (x,y) \in S].$
    %\item For any sets $S, T \subseteq [q]^n$, we write $\mu_{\mid S \times T}$  for the distribution $\mu$ conditioned on $(x,y) \in S \times T$.
\end{itemize}
\ignore{
\begin{center}
  \fbox{\begin{minipage}{\textwidth}
  \paragraph{Preliminaries and Notation}
 \begin{itemize}
 	\item We use distributions, densities and random variables interchangeably with the meaning being clear from the context.
    \item For a random variable $Y$ on $\on^{bn}$, a block of variables $I \subseteq [n]$ and $\alpha \in \on^{bI}$, we write $(Y \mid Y_I = \alpha)$ for the random variable $Y$ conditioned on the event $Y_I = \alpha$.
    \item For $\mu$, a density on $\on^{bn} \times \on^{bn}$, and any subset $R \subseteq \on^{bn} \times \on^{bn}$, we write $\mu(R)$ for $\Pr_{(x,y) \sim \mu}[ (x,y) \in R].$
    \item For any sets $X, Y \subseteq \on^{bn}$, we write $\mu_{\mid X \times Y}$  for the distribution $\mu$ conditioned on $(x,y) \in X \times Y$.
\end{itemize}
  \end{minipage}}
\end{center}}

\ignore{ Commented Out in Red:  In case, we need something from here
\subsubsection{Conjunctive Blockwise Denseness and Junta Approximation}

%As before, we view $\on^{bn}$ as a collection of strings each of which consists of $n$ disjoint blocks of $b$ bits each. For a random variable $X$ on $\on^m$ and any $I \subseteq [n]$, we write $X_I$ for the random variable that ignores all but the blocks indexed by $i \in I$.

We begin with \emph{blockwise dense} densities. These are random variables on $[q]^{n}$ such that the marginal on any sub-collection of blocks has high min-entropy. Intuitively, they are our versions of ``almost uniform'' densities.
\begin{definition}[Blockwise Dense Random Variables]
A random variable $X$ on $[q]^{n}$ is said to be $S$-blockwise dense for $S \subseteq [n]$ if for every $I \subseteq S$, $H_{\infty}(X_{I}) \geq (0.8 \cdot \log{q}) \cdot |I|.$ $X$ is said to be blockwise dense if it is $[n]$-blockwise dense.
\end{definition}

The central motivation behind the definition of {\it block-wise dense} random variables is the following observation, first made in \cite{GLMWZ15}.
%
\begin{lemma}\label{lem:bd-epsilon-decay}
Fix $q = 2^b$ for $b > 7$ and identify $[q]$ with $\on^b$.  Let $\iproduct : \on^b \times \on^b \to \on$ be the boolean inner product function.

Suppose $X$ and $Y$ are independent, blockwise dense random variables in $[q]^{n}$. Let $\nu$ be the density of the random variable $\iproduct^{\otimes n} (X,Y)$ on $\on^n$. Then, $\nu = 1 + h$ for an an $\epsilon$-decaying function $h$ where $\epsilon =  2^{-0.5b}.$ \label{lem:bd-epsilon-decay}
\end{lemma}
%
The lemma is an easy consequence of the properties of $2$-bit inner product, of which the most important being that it is a $2$-source extractor \cite{CG88}.  We begin by formally recalling this fact.
%We will need the following fact in the proof. Recall that $g$ is the $b$ bit Boolean inner product function with outputs in $\on$.

\begin{fact}[Chor-Goldreich \cite{CG88}]
Suppose $X, Y $ are independent random variables over $\on^{\ell}$ for $\ell > 7$ with min-entropy $H_{\infty}(X),H_{\infty}(Y) \geq 0.8 \ell$. Then, for the boolean inner product function $\iproduct$,
\[|\Pr[ \iproduct(X,Y) = +1 ]-\half|  \leq 2^{-0.6 \ell} \mcom\]
or equivalently,
\[|\E[\iproduct(X,Y)]| \leq 2^{-0.8 \ell + 1} \mper \]
\label{fact:Chor-Goldreich}
\end{fact}

% \begin{fact}[Chor-Goldreich \cite{CG88}]
% Suppose $X, Y $ are independent, blockwise dense random random variables over $\on^{bn}$ for $b > 7$. Then, for any $I \subseteq [n]$, $|\Pr[ \Pi_{i \in I} g(X_{\{i\}},Y_{\{i\}}) = +1 ] - 1/2| \leq 2^{-0.8b|I|}.$  \label{fact:Chor-Goldreich}
% \end{fact}
\begin{proof}[Proof of Lemma \ref{lem:bd-epsilon-decay}]
Observe that using Fact \ref{fact:Chor-Goldreich}, for any $S \subseteq [n]$ we have
\[ \hat{\nu}(S) = \E[ \nu(z) \chi_S(z)] = \E_{z \sim \nu}[ \chi_S(z)] = \E[\Pi_{i \in I} g(X_{\{i\}},Y_{\{i\}})] = \E[\iproduct(X_{S},Y_{S})] \leq 2^{-0.8b|S|+1}.\]

Let $h(z) = \sum_{|S| \geq 1} \hat{\nu}(S) \chi_S(z).$ Then, $\nu = 1 + h$ and by the above estimate, $h$ is $\epsilon$-decaying for $\epsilon = 2^{-0.8b} \leq 2^{-0.5b}.$
\end{proof}


A conjunctive blockwise dense random variable is one for which there is a small subset of blocks that are ``fixed'' (and thus has $0$ entropy) while the the marginal distribution on the remaining blocks is blockwise dense.  Formally, conjunctive block-wise dense random variables are defined as follows.

\begin{definition}[$d$-\cbd and aligned $d$-\cbd pairs]
A random variable $X$ on $[q]^{n}$ is $d$-\emph{conjunctive blockwise dense} ($d$-\emph{\cbd}) if there exists a set of coordinates $I \subseteq [n]$, $|I| \leq d$ such that $H_{\infty}(X_I) = 0$ and for every $J \subseteq [n]\setminus I$, $H_{\infty}(X_J) \geq (0.8 \cdot \log_2 q)
 \cdot |J|.$ The set of coordinates $I$ are the \emph{fixed blocks} of $X$.

We say that two random variables $X$ and $Y$ with $d$-\cbd densities on $[q]^{n}$ are \emph{aligned} if they have the same set of fixed blocks.
\end{definition}

By Lemma \ref{lem:bd-epsilon-decay}, if $X,Y$ are $\bd$ random variables, then the density of the $\iproduct^{\otimes n}(X,Y)$ is an $\epsilon$-decaying perturbation of the uniform density. In the following, we show a refinement of Lemma \ref{lem:bd-epsilon-decay} when $X,Y$ are aligned $d$-$\cbd$ random variables - specifically, that $\iproduct^{\otimes n}(X,Y)$ is a an $\epsilon$-decaying perturbation of a non-negative $d$-junta.

\begin{lemma}
Fix $q = 2^b$ and identify $[q]$ with $\on^b$.

Let $X,Y$ be aligned $d$-$\cbd$ random variables over $[q]^n$ for $b > 7$ with the aligned blocks $I \subseteq [n]$ and $X_I = \alpha, Y_I = \beta$. Let $\nu$ be the density of $z = \iproduct^{\otimes n}(X,Y).$ Then, for $\epsilon  = 2^{-0.5b}$, there exists an
$\epsilon$-decaying function $h$ such that
%
\[\nu = 2^{|I|} \cdot \1[z_I = \iproduct^{\otimes |I|}(\alpha, \beta)] \cdot (1+h).\] \label{lem:junta-approx-for-CBD}
\end{lemma}
\PRnote{For events and indicator of events, I like $\1[E]$ over $\1(E)$}

\pnote{use a standard symbol for the gadget g}

\PRnote{need a consistent notation for gadget $g$,and its special case, $\iproduct$.  I have chosen one here, hopefully we can find something better}
\begin{proof}
Observe that $z_{I} = \iproduct^{\otimes |I|}(\alpha, \beta)$ and $z_{\bar{I}} = \iproduct^{\otimes |\bar{I}|}(X_{\bar{I}}, Y_{\bar{I}})$. Since $X_I = \alpha$ and $Y_I = \beta$ are fixed, we have that $z_I$ is fixed as $z_I = \iproduct^{\otimes |I|}(\alpha, \beta).$ In particular, the density of $z$ can be written as $\nu_I \cdot \nu_{\bar{I}}$ where $\nu_I$ is the  density of $z_I$ and $\nu_{\bar{I}}$ the density of $z_{\bar{I}}$.

Now, by definition, $X_{\bar{I}}, Y_{\bar{I}}$ are $d$-$\cbd$ random variables and thus, the density $\nu_{\bar{I}}$ of $z_{\bar{I}}$ can be written as $1+h$ for an $\epsilon$-decaying function for $\epsilon = 2^{-0.5b}$ using Lemma \ref{lem:bd-epsilon-decay}. This completes the proof.
\end{proof}

}

\subsection{Warm Up: One-Dimensional Decompositions}

%As a warm up,  we show a simple short argument that any high entropy density can be decomposed into a convex combination of densities each of which are \cbd.
%
%In the next section, we prove Theorem \ref{thm:maindecomp} which requires a much more subtle argument.

Observe that by definition, any $d$-\cbd density has min-entropy at least $0.8 \log q (n-d)$ which for $d \ll n$, we consider high. Thus, any convex combination of $d$-\cbd densities also has high min-entropy.
%
One could ask for a converse at this point: can every high min-entropy density be written as a convex combination of $d$-\cbd densities for small $d$? As a warmup for the more general decomposition, we first show that this is indeed the case. 

%In this section, as a warmup, we show that the answer is indeed yes.


\begin{lemma} \label{lem:warmup-single-density}
Let $\mu$ is a density on $[q]^{n}$ with $H_\infty(\mu) \geq (n - t) \cdot \log q$.  Then, there exists a partition of $[q]^n$ as
\[[q]^n = \left(\bigcup_{i \in [N]} S_i\right) \cup S_{err} \]
such that
\begin{itemize}
\item For each $i \in [N]$, $\mu_{ \mid S_i}$ is a $20t$-\cbd distribution.
\item $\mu(S_{err}) \leq q^{-t}$.
\end{itemize}
\end{lemma}
\begin{proof}
We present an algorithm that obtains the claimed partition.

\begin{center}
  \fbox{\begin{minipage}{\textwidth}

  \textit{Setup:} $\mu$ is a distribution over $[q]^n$ with $H_{\infty}(\mu) \geq (n-t) \cdot \log q$. Fix $t' = 2t$.\\

  \textbf{Decompose(S)}\\
  \textit{Input} $S \subseteq [q]^n$. 
\begin{enumerate}
\item If $\mu_{|S}$ is \bd \textsc{Terminate} and return $S$.
\item If $H_\infty(\mu_{|S}) \leq (n-t') \cdot \log q$, \textsc{Terminate} and return $S$, labeled as \textsc{Error}.
\item Else, let $Y \sim \mu_{|S}$.  Let $I \subseteq [n]$ be a \emph{maximal} set such that $H_\infty(Y_I) < 0.8 \log q  \cdot |I|$ and suppose $\alpha \in [q]^{I}$ be such that $p = \pr_{\mu_{|S}}[Y_I = \alpha] \geq q^{-0.8 |I|}$. Then, set $S_1 \lfta S \cap \{y \in [q]^n: y_I = \alpha\}$ and $S_2 \lfta S \cap \{y \in [q]^n: y_I \neq \alpha\}$.
%Then, $Y_1$ is blockwise-dense.
\item \textsc{Return} $S_1 \cup  \textsc{Decompose}(S_2)$.
\end{enumerate}
  \end{minipage}}
\end{center}
%
To get the desired decomposition of $\mu$, we call $\textsc{Decompose}([q]^n)$.
%
Observe that the algorithm returns a partition of $[q]^n$ into subsets $\{S_i\}_{i \in [N]}$ (constructed in Step (3) or Step (1) ) and possibly a subset $S_{err}$ labeled {\sc ERROR} (if the algorithm terminates via Step (2)).

First, we claim that for the sets $S_i$ constructed in step (3) of the algorithm, the corresponding distributions $\mu_{|S_i}$ are $d$-\cbd for $d = 10t'$.  Consider any execution of the Decompose routine that generates sets $S_1,S_2$ in Step (3).  Since $I$ is a maximal set such that $H_{\infty}(Y_I) < 0.8 \log q |I|$, for any subset $J \subseteq [n]\slash I$, we have $H_{\infty}(Y_{J} | Y_{I} = \alpha) > 0.8 \log q |J|$, i.e., $Y|Y_{I} = \alpha$ is block-wise dense except for the fixed coordinates in $I$. Further, if the execution did not terminate in Step (2), then $H_{\infty}(\mu_{|S}) \geq (n-t') \cdot \log q$, i.e.,  $\Pr_{\mu_{|S}}[Y = \beta] \leq q^{t'} \cdot q^{-n}$ for all $\beta \in [q]^n$.  Therefore we have,
\[ q^{-0.8 |I|} \leq \Pr_{\mu_{|S}}[Y_{I} = \alpha] \leq q^{n-|I|} \cdot \max_{\beta \in [q]^n} \Pr_{\mu_{|S}}[Y = \beta]  \leq  q^{t' - |I|} \mcom \]
which implies that $|I| \leq 5 t'$.  We have argued that all distributions produced by the algorithm are $5t'$-\cbd, except for the error term $S_{err}$.

By Step(2), the distribution $\mu_{|S_{err}}$ labeled as \textsc{Error} has min-entropy  $H_{\infty}(\mu_{|S_{err}}) \leq (n-t') \cdot \log q = (n-2t) \cdot \log q$.  Since $H_{\infty}(\mu) \geq (n-t) \cdot \log q$, this implies that $\mu(S_{\err}) \leq q^{t-t'} = q^{-t}.$

\end{proof}
\subsection{Rectangular Decompositions}
To prove our junta theorem, \prettyref{thm:mainjunta}, and for other plausible applications in communication complexity, the decomposition obtained by  \prettyref{lem:warmup-single-density} does not suffice.  In particular, the underlying domain is two-dimensional $[q]^n \times [q]^n$, and the partitions need to be {\it rectangular}.  In this section, we will prove a general {\it rectangular decomposition} theorem designed for distributions with high min-entropy.

%The setup is as follows.
%Let us denote $b \defeq \log q$.

A combinatorial rectangle $\cR \subseteq [q]^n \times [q]^n$ is given by $\cR =  \cA \times \cB$ for $\cA,\cB \subseteq [q]^n$. We can now state our main decomposition theorem. \ignore{For a density $\mu$, we will denote by $\mu_{|R}$ the density $\psi$ conditioned on being within $R$, i.e.,
\[\mu_{|R}(x,y) = \mu(x,y) \cdot \frac{\Ind[ x \in \cA \wedge y \in \cB ] }{\mu(R)} \mcom\]
where $\mu(R)$ is total probability mass of $\mu$ within $R$, namely $\mu(R) = \Pr_{\mu}[ x \in \cA \wedge y \in \cB]$.}


\begin{theorem}[Rectangular Decompositions]\label{thm:maindecompfull}

Let $\mu$ be a probability density on $[q]^n \times [q]^n$ such that for all $I \subseteq [n]$,
\[ H_{\infty}(\mu_{I}) \geq 1.9 \cdot \log{q} \cdot |I| - t \mper\]
Then for all $d \in \N$, there exists a partition
\[ [q]^n \times [q]^n = \left(\bigcup_{i \in [N]} \cR_i \right)\cup \Error\] where $\{\cR_i = \cA_i \times
\cB_i\}_{i \in [N]}$ are rectangles such that
\begin{enumerate}
\item For each $i \in [N]$, $(X_i,Y_i) \sim \mu_{\mid \cR_i}$, $X_i,Y_i$ are aligned $d$-$\cbd.$
\item $\mu(\Error) \leq 2^t \cdot (dq^{-0.05})^d$
\end{enumerate}
\label{thm:alg-analysis}
\end{theorem}

Notice that the above theorem also implies that the density $\mu$
can be approximated by a convex combination of aligned $d$-\cbd distributions
by setting,
\[ \mu = \sum_{i \in [N]} \mu(\cR_i) \cdot \mu_{|\cR_i} + \mu(\Error)
\cdot \mu_{|\Error} \mper\]
%
\prettyref{thm:maindecomp} is an an immediate consequence of the above decomposition theorem.  
\begin{proof}[Proof of \prettyref{thm:maindecomp}]
Let $\mu$ be the density $u \otimes v$ on $[q]^n \times [q]^n$. Then, $\mu$ for all $I \subseteq [n]$, $H_\infty(\mu_I) \geq 2 (\log q) |I| - t$.  Now, apply \prettyref{thm:maindecompfull} to obtain a partition of $[q]^n \times [q]^n$ as $\cup_{i \in N} \cR_i \cup \Error$ satisfying the conditions of the theorem. Then,
$$\mu = \sum_{i=1}^N \mu(\cR_i) \cdot \mu_{|\cR_i} + \mu(\Error) \mu_{|\Error}.$$
Note that $\sum_{i=1}^N \mu(\cR_i) + \mu(\Error) = 1$.
Let $\cR_i = \cA_i \times \cB_i$. Then, we can write $\mu_{|\cR_i} = u_i \otimes v_i$, where $u_i = u_{|\cA_i}$ and $v_i = v_{|\cB_i}$. Then, $X_i \sim u_i, Y_i \sim v_i$ are aligned $d$-\cbd and 
$$\mu(\Error) \leq 2^{t} (dq^{-0.05})^d \leq 2^{-t} (nq^{-0.05})^d \leq 2^{-t} q^{-\Omega(d)} \leq q^{-\Omega(d)},$$
for $q \geq n^c, d \geq c t$ for a sufficiently big constant $c \geq 1$. This proves the theorem.
\end{proof}
%\PRnote{do we need a proof?}
%We include the proof below for the sake of completeness.
%
%\begin{proof}[Proof of \prettyref{thm:maindecomp}]
%	\PRnote{need to fix the statement of thm:maindecomp, will get to it after commit}
%\end{proof}



\subsection{The Decomposition Algorithm}\label{sec:decompalgorithm}

We will show \prettyref{thm:alg-analysis} by devising an algorithm
that constructs the partition given the distribution $\mu$ and a
parameter $d \in \N$. The algorithm is an natural extension of the one used in the proof of \prettyref{lem:warmup-single-density} and is similar to the one used in \cite{GLMWZ15}; however, our analysis is quite different from theirs. Indeed, while they also obtain a similar decomposition theorem, the error guarantee is not exponentially small as we obtain and is needed in our application.  

The formal description of the algorithm is at the end of this
subsection. For exposition, we depict a labeled execution tree of the
algorithm \prettyref{fig:exec-tree}. \Dec is the main procedure that takes as input a rectangle $\cA \times
\cB \subseteq [q]^{n} \times [q]^{n}$. This rectangle will always satisfy the invariant of
having an \emph{aligned} set of nodes \emph{fixed} - i.e. there is an
explicitly identified set of indices $F \subseteq [n]$ such that for some two fixed strings $\alpha, \beta$, for all $(x,y) \in \cA \times \cB$, $x_F = \alpha$ and $y_F = \beta$. Observe that in the beginning, $\cA = \cB = [q]^{n}$ and $F = \emptyset.$

Each time $\Dec$ is invoked by the algorithm, we create a new node in the execution tree and identify it as being created by $\Dec$ by indexing it with $v_1, v_2, \ldots, $. If the set of fixed blocks $F$ in the input rectangle $\cR$ has size $\geq d$, the algorithm terminates and adds the associated rectangle $\cR$ to $\Errorb$; $\Errorb$ contains the set of rectangles that account for error owing to the number of fixed blocks in them exceeding $d$.  Next, if $\mu(\cR) < \delta$, then $\cR$ is added to $\Errora$; $\Errora$ maintains the collection of rectangles that are labeled as error because their measure was too small.

Now, suppose that the input rectangle $\cR$ does not satisfy the conditions of $\Errora$ or $\Errorb$. If $\mu_{\mid \cR}$ is $\bd$, then, we terminate the algorithm and return $\cR$. Otherwise, there exists $S \subseteq [n]$ and some assignment to variables in $S$, say $\alpha_S$ such that $\Pr_{\mu_{\mid \cR}}[ X_S = \alpha_S ] > q^{-0.8|S|}$ (or $\Pr_{\mu_{\mid \cR}}[ Y_S = \alpha_S] > q^{-0.8|S|}).$  The idea is to split the rectangle $\cA \times \cB$ into two rectangles, $\cA_{|S = \alpha_S} \times \cB$ and $\cA_{|S \neq \alpha_S} \times \cB$; here, we define $\cA_{|S = \alpha_S}$ denotes the set,
\[ \cA_{|S = \alpha_S} = \cA \cap \{x: x_{S} = \alpha_S\} \text{ and } \cA_{|S \neq \alpha_S} = \cA \cap \{x: x_{S} \neq \alpha_S\}\mper  \]
In the rectangle $\cA_{|S = \alpha_S} \times \cB$, $X$ and $Y$ don't have the same set of fixed blocks, since $X$ is fixed in $F \cup S$ while $Y$ is fixed only on $F$.  
%
To remedy this, the subroutine $\XDec$ (or $\YDec$, respectively) is executed on the rectangle $\cA_{|S = \alpha_S} \times \cB$.  The \Dec routine continues with the remaining rectangle $\cA_{\mid S \neq \alpha_S} \times \cB$.  Each call to $\XDec$ or $\YDec$ is denoted by a node in the execution tree labelled by $w_1, w_2, \ldots.$ 

The subroutine $\XDec$ (the case of $\YDec$ is analogous) takes as input the rectangle $\cA \times \cB$ along with the fixed set $F$ that was the current input of the $\Dec$ routine when $\XDec$ was invoked in addition to the new set of indices $S$ that violated blockwise-density. $\XDec$ then chooses every possible value $\beta$ for $Y_S$ and for each $\beta$, calls $\Dec$ recursively with the rectangle $\cA \times \cB_{\mid S = \beta}$ with $F \cup S$ as the set of fixed coordinates.

\begin{center}
  \fbox{\begin{minipage}{\textwidth}
  \captionof*{figure}{Decomposition Algorithm}
  \label{alg:dec}
  \textit{Setup:} \begin{itemize}\itemsep=0ex
		  \item           A probability density $\mu$ such that  $ H_{\infty}(\mu_{\mid I}) \geq 1.9 \log{q} \cdot |I| - t$ for all $I \subseteq [n]$. 
     \item A parameter $d \in \N$ and let $\delta \defeq q^{-0.05d}$. Set $\Errora = \Errorb = \emptyset$.
                  \end{itemize}
\textbf{Decompose$(\cA \times \cB,F)$}\\
\textit{Input:}   A rectangle $\cA \times \cB \subseteq [q]^n \times [q]^n$, $F \subseteq [n]$: subset of ``fixed'' indices.  \\
  \textit{Invariant:} $\cA_F,\cB_F$ are fixed.
\begin{enumerate}
%\item Initialize $\Errorb, \Errora \leftarrow \emptyset.$
\item If $|F| \geq d$, \textsc{Terminate} after setting $\textsc{Error}_d \lfta \textsc{Error}_d \cup \cA \times \cB$.
\item Set $\cR \equiv \cR_0 \equiv \cA \times \cB$.
\item While $\mu(\cR) \geq \delta \cdot \mu(\cR_0)$ do
	\begin{enumerate}
		\item Let $(X,Y) \sim \mu_{|\cR}$. If $X_{\overline{F}}, Y_{\overline{F}}$ are $\bd$, \textsc{Terminate}.
        \item Else, if there is an $S \subseteq [n] \backslash F$ and $\alpha \in [q]^S$ such that
				$$ \Pr[X_S = \alpha] > q^{-0.8  |S|},$$ call $\YDec$ on input $(\cA_{|S=\alpha},\cB,F,S)$ and set $\cR \leftarrow \cA_{|S \neq \alpha} \times \cB$

	 	\item Else, if $\Pr[Y_S = \alpha] > q^{-0.8  |S|}$ then call $\XDec$ on input $(\cA,\cB_{|S = \alpha},F,S)$ and set $R \leftarrow \cA \times \cB_{|S \neq \alpha}$.
	\end{enumerate}
\item Set $\Errora \leftarrow \Errora \cup R$.
\end{enumerate}
  \end{minipage}}

  \fbox{\begin{minipage}{\textwidth}
  \textbf{XDecompose$(\cA \times \cB, F, S)$} \\
 \textit{Input:} A rectangle $\cA \times \cB$, $F \subseteq [n]$: common subset of
 ``fixed'' indices; $S$: the set of coordinates newly fixed in $\cA$ (but not in $\cB$).\\
  \textit{Invariant:} $X_{F}$ and $Y_{F \cup S}$ are fixed.
  \begin{enumerate}
  	\item For every $\beta \in [q]^S$,
		\textsc{Decompose}$(\cA_{|S = \beta},\cB,F\cup S)$.
  \end{enumerate}

  \end{minipage}}

  \fbox{\begin{minipage}{\textwidth}
  \textbf{YDecompose$(\cA \times \cB, F,S)$} \\
   \textit{Input:} A rectangle $\cA \times \cB$, $F \subseteq [n]$: common subset of ``fixed'' indices. \\
  $S$: the set of coordinates newly fixed in $\cB$ (but not in $\cA$). \\
  \textit{Invariant:} $X_{F \cup S}$ and $Y_F$ are fixed.
  \begin{enumerate}
  	\item For every $\beta \in [q]^S$,
		\textsc{Decompose}$(\cA,\cB_{|S=\beta},F\cup S)$.
  \end{enumerate}

  \end{minipage}}


\end{center}

\begin{figure}[h]
\begin{center}
\includegraphics[scale=0.50]{tree-diagram.pdf}
\caption{Execution Tree: Blue Nodes are Calls of $\Dec$, Red Nodes are calls of $\XDec$ or $\YDec$. ``too deep"  $\equiv \Errora$, ``too small'' $\equiv \Errorb$ and BD = $\bd$}
\end{center} \label{fig:exec-tree}
\end{figure}

%The following is the main claim that captures the relevant claims about the algorithm.


\subsection{Analysis:Proof of \prettyref{thm:alg-analysis}}
%In the following, we analyze the procedure above.
We now analyse the algorithm. 

\paragraph{Execution Tree} Consider the execution tree of the decomposition algorithm  (Figure \ref{fig:exec-tree}). We associate a node $\rho$ corresponding to a call of $\Dec$ with parameters $\cA_\rho, \cB_\rho$ and $F_\rho$ for $\cA_\rho, \cB_\rho \subseteq [q]^n $ and $F_\rho \subseteq [n].$ Nodes $\rho$ corresponding to a call of $\XDec$ or $\YDec$ are associated with an additional parameter $S_\rho \subseteq [n]$. The calls of $\Dec$ and $\XDec$ or $\YDec$ alternate.

Before we analyze the decomposition, we introduce some notation.
\newcommand{\depth}{\mathsf{depth}}
\begin{itemize}
\item For each vertex $\rho$, let $\mu(\rho) = \mu(\cA_{\rho} \times \cB_\rho)$.  Let $R(\rho)$ denote the rectangle $\cA_{\rho} \times \cB_{\rho}$.
%\item The $\depth(\rho)$ of any node $\rho$ in the tree is the number of edges on the path from root to $\rho.$
\item For a child $b$ of a vertex $a$, let $\mu(b|a) = \mu(b)/\mu(a)$.
%- the conditional probability of traversing the edge $(a,b)$ in the tree when at vertex $a$.

\item We will reserve the letter $v$ (and various suffixes) for nodes corresponding to calls of $\Dec$ (i.e., the vertices in odd-layers) and the letter $w$ for nodes corresponding to calls of $\XDec$ or $\YDec$ (i.e., the vertices in even-layers).

\item For a vertex $v$ let $C_v = (w_1,\ldots,w_{c_v})$ be the children of $v$ (in the order they were generated), where we assume that $w_1,\ldots,w_{c_v-1}$ lead to recursive calls of $\XDec$ or $\YDec$ while $w_{c_v}$ corresponds to the rectangle marked as $\Errora$ in Step(4) of $\Dec$.

\item For a vertex $v$, and $w_i \in C(v)$, let $S_{w_i} \subseteq [n]$ denote the corresponding set of new blocks that were fixed to produce $w_i$.

\item We say a node $v$ in the tree is {\it bad} if $|F_v| \geq 2d$ but $\mu_{|\cA_{v}\times \cB_{v}}$ is not \bd in the non-fixed blocks.  A root-to-leaf path $v_1,w_1,v_2,w_2,\ldots,
	v_t, w_t,v_{t+1}$ is called a {\it bad path} if $v_{t+1}$ is bad.
\end{itemize}

Note that the tree yields a partition of $[q]^n \times [q]^n$ as,
\[ [q]^n \times [q]^n = \left(\bigcup_{v \in \cL]} \cR(v) \right)\cup \Errora \cup \Errorb,\]
where $\cL$ denotes the leaves of the tree not added to $\Errora$ or $\Errorb$. We will show that this partition satisfies the conditions of the theorem when we take $\Error = \Errora \cup \Errorb$. Note that, all the leaves in the execution tree correspond to the calls of $\Dec$. 

We first argue that $\mu_{|\cR(v)}$ for $v \in \cL$ gives $d$-$\cbd$ densities in the non-fixed coordinates. % and further, if for such a leaf $v$, the corresponding rectangle $R(v)$ is not added to $\Errora$ or $\Errorb$ at any point, then $\mu_{|R}$ is $d$-$\cbd$. We record this observation as the following fact:

\begin{lemma}[Good Rectangles]
Let $v \in \cL$. Then, $\mu_{\mid \cR(v)}$ is an aligned $d$-$\cbd.$ \label{lem:proof-part-1}
\end{lemma}
\begin{proof}
The assumptions imply that $|F_v| \leq d$. Further, as $\cR(v)$ was not added to $\Errora$, $\cR(v)$ is a leaf because for $(X,Y) \sim \mu_{\mid \cR(v)}$, $X_{\bar{F}}, Y_{\bar{F}}$ are $\bd$. Thus, $\mu_{\mid \cR(v)}$ is an aligned $d$-$\cbd$ denisty. 

%Since $\cR(v)$ is not added to $\Errora$, $\cR(v)$ is a leaf because $\mu_{\mid R}$ is $\bar{F}$-blockwise dense or equivalently, $\mu_{\mid R}$ is $d$-$\cbd$.
\end{proof}

It is also easy to bound $\mu(\Errora)$:

\begin{lemma}
$\mu(\Errora) \leq d \delta.$ \label{lem:proof-part-2}
\end{lemma}

\begin{proof}
Note that each call of \textsc{Decompse} leads to at most one rectangle being added to $\Errora$. Further, if $\textsc{Decompse}(R_0)$ led to adding a rectangle $\cR \subseteq \cR_0$ to $\Errora$, then $\mu(R) < \delta \cdot \mu(R_0)$. Now, in any single layer of the execution tree the nodes corresponding to calls of $\Dec$ are associated with disjoint rectangles. Thus, the total measure of all the rectangles that are included in $\Errora$ due to $\Dec$ calls from nodes in a specific layer is at most $\delta$. As there are at most $d$ layers that have $\Dec$ nodes, it follows that $\mu(\Errora) \leq d \delta$.% There are at most $d$ layers that have $\Dec$ nodes that could lead to children that are included in $\Errora$. Thus, $\mu(\Errora) \leq d\delta$
\end{proof}

The main task is to prove an upper bound on $\mu(\Errorb)$.
\paragraph{Bounding $\mu(\Errorb)$}

We begin with an important definition. 

\begin{definition}[$\theta(w_i \mid v)$]
For a node $v$ associated with a $\Dec$ call, let $C_v = (w_1,\ldots,w_{c_v})$ be the children of $v$. Define 
$$\theta(w_i \mid v) = \sum_{j=i}^{c_v} \mu(w_j \mid v).$$ 
\end{definition}
Intuitively, $\theta(w_i \mid v)$ denotes the relative measure of the rectangle $\cR$ inside Step $4$ of Algorithm \ref{alg:dec} just before the call of $\XDec$ or $\YDec$ associated with the node $w_i$. 

\ignore{Let $w_i$ be the child associated with the $i^{th}$ call of $\XDec$ or $\YDec$ inside the call of $\Dec$ associated with some node $v$.

\begin{definition}[$\theta(w_i \mid v)$]
Let $\theta(w_i \mid v)$ denote the relative measure under $\mu$ of the rectangle $R$ inside Step $4$ of Algorithm \ref{alg:dec} just before the call of $\XDec$ or $\YDec$ associated with the node $w_i$.
\end{definition}

$\theta(w_i \mid v)$ can be expressed in terms of $\mu$ as follows:

\begin{lemma}[Measure at $w$ Nodes]
Let $w_1, w_2, \ldots,$ be the $w$-nodes that are children of $v$ in the execution of the algorithm. Then,
$$\theta(w_i|v) = \sum_{j=i}^{c_v} \mu(w_j|v).$$\label{lem:def-theta}
\end{lemma}
\begin{proof}
Let $R_i$ be the rectangle that step 4 of $\Dec$ works with just before the call of $\XDec$ or $\YDec$ that creates the node $w_i.$ Each iteration of the while loop in step 4 of the algorithm further partitions $R$. The total $\mu$-measure of $R_i$ can thus be obtained by summing up the measures of all the rectangles $R_j$ that occur in $\Dec$ at $v$ at or after the call of $\XDec$ or $\YDec$ that creates $w_i.$
\end{proof}}



% \begin{lemma} \label{lem:partition}
% 	For each vertex $v$, the family of sets $\{X_w \times Y_w \mid w \in C(v) \}$ forms a partition of
% 		$X_{v} \times Y_{v}$. In particular, $\mu(v) = \sum_{w \in C_v} \mu(w)$.
% \end{lemma}
% \begin{proof}
% 	Easy.
% \end{proof}

\begin{lemma}\label{lem:density}
Fix any vertex $v$ and a child $w$ of $v$,
$$\mu(w|v) \geq q^{-0.8 |S_w|} \cdot \theta(w|v).$$
\end{lemma}
\begin{proof}
Let $\cR$ be the rectangle processed in the while loop inside the call of $\Dec$ associated with $v$ just before the call to create $w$. Suppose that $w$ was created by a recursive call to $\XDec$ for $S_w \subseteq [n]$ such that $\Pr_{(X,Y) \sim \mu_{|\cR}}[ X_{S_w} = \alpha] \geq q^{-0.8 |S_w|}$ (the case of a call to $\YDec$ can be dealt with analogously). Thus, $\mu_{|\cR}(\cR(w)) \geq q^{-0.8 |S_w|}$.

Now, we can write  $\mu(w | v) $ as a product of the relative probability of $\cR$ in $\cR(v)$ and the relative probability of $\cR(w)$ under $\cR$. Concretely, 
$$\mu(w | v) = \mu_{|\cR(v)}(\cR(w)) = \mu_{|\cR(v)}(\cR) \cdot \mu_{|\cR}(\cR(w)) = \theta(w|v) \cdot \mu_{|\cR}(\cR(w)) \geq \theta(w |v) \cdot q^{-0.8 |S_w|},$$
where the last equality follows from the definition of $\theta(w|v)$. 

%But $\mu(w \mid v) = \mu(w \mid R) \mu(R \mid v).$ By definition, $\theta(w \mid v)$ is the relative measure of $R$ inside $R(v)$, i.e., $\mu(w|R) = \theta(w|v)$.  Thus, $\mu(w \mid v) \geq q^{-0.8  |S|} \mu(R \mid v) = q^{-0.8  |S_w|} \theta(w \mid v).$


% Let $w$ be the $i$'th child of $v$ and let $R_i$ denote the rectangle in the iteration when $w_i$ was created. Then, $\mu(R_i) = \sum_{j=i}^{c_v} \mu(w_j) = \theta(w|v) \mu(v)$. Further, by Step 4(b) (or 4(c)),
% $$\frac{\mu(w|v)}{\theta(w|v)} =  \frac{\mu(w)}{\mu(R_i)} \geq 2^{-0.8 b |S_w|}.$$
\end{proof}

Next, we estimate $\mu(v)$ for every $v$ that is a \emph{bad} leaf i.e., a leaf at depth $2d+1.$  We begin by showing a bound on $\mu(v)$ for an arbitrary node $v$.
\begin{lemma} \label{lem:node-measure-bound}
For any vertex $v$ in the execution tree,
\[ \mu(v) \leq 2^t \cdot q^{- 1.9 |F_v|} \mper\]
%where $F_v$ is the set of fixed blocks at vertex $v$.
\end{lemma}
\begin{proof}
	The rectangle $\cR(v)$ corresponding to $v$ has the blocks $F_v$ fixed, while the values in the remaining blocks could also be constrained.  Let us suppose $X_{F_v} = \alpha$ and $Y_{F_{v}} = \beta$ for $(X,Y) \in \cR(v)$.  By our assumption on $\mu$,
\[ H_{\infty}(\mu_{|F_v}) \geq 1.9 \cdot \log q \cdot |F_v| - t \mcom\]
which implies that,
\[ \mu(v) \leq \Pr_{\mu} [X_{F_v} = \alpha \wedge Y_{F_v} = \beta ] \leq 2^{-H_{\infty}(\mu_{F_v})} \leq 2^t \cdot q^{-1.9 |F_v|} \mper\]
\end{proof}


\begin{lemma}\label{lem:badleafbound}
Let $v_1,w_1,\ldots, v_\ell,w_\ell,v_{\ell+1}$ be a {\emph bad} path ending at a node that is added to $\Errorb$. Then,
	$$\mu(v_{\ell+1}) \leq q^{-1.1 |F_{v_{\ell+1}}|} \cdot 2^t  \cdot
	\prod_{i=1}^{\ell} \frac{\mu(w_i|v_i)}{\theta(w_i | v_i)}
	$$ \label{lem:bad-path-prob}
\end{lemma}

\begin{proof}
Let $s = |F_{v_{\ell+1}}|$; then, by \prettyref{lem:node-measure-bound},
	\begin{align*}
    \mu(v_{d+1}) & \leq q^{-1.9 s} \cdot 2^t
    \end{align*}
%	$$\mu(v_{d+1}) \leq q^{-2s} \cdot 2^{t}.$$

On the other hand, we know that $\sum_{i=1}^\ell |S_{w_i}| = s$. Thus, by \lref{lem:density},
    $$
	\mu(v_{\ell+1}) = \prod_{i = 1}^\ell \mu(v_{i+1}|w_i) \mu(w_i |
	v_i)
	\geq \prod_{i = 1}^\ell \mu(v_{i+1}|w_i) \cdot \theta(w_i |
	v_i) \cdot q^{-0.8  |S_{w_i}|}.
$$ The above two
	inequalities imply that,
	$$ \prod_{i=1}^\ell \mu(v_{i+1}|w_i) \theta(w_i | v_i) \leq
	q^{-1.1 s} \cdot 2^t.$$

	The claim now follows from the above
	inequality along with
	$$\mu(v_{\ell+1}) = \prod_{i=1}^{\ell}
	\mu(v_{i+1}| w_{i}) \mu(w_i | v_i)  = \bkets{\prod_{i=1}^\ell \mu(v_{i+1}| w_i) \theta(w_i | v_i)} \cdot \prod_{i=1}^\ell \frac{\mu(w_i | v_i)}{\theta(w_i | v_i)}.$$

\end{proof}

We need the following elementary lemma.
\begin{lemma}
	Let $a_1,\ldots, a_N \in (0,1) $ be such that $\sum_{i = 1}^{N} a_i = 1$ and $a_{N-1} + a_N \geq \eps$. % for every $i < N$, $\sum_{j \geq i} a_j > \epsilon$. 
	Then,
	$$ \sum_{j = 1}^{N} \frac{a_j}{ \sum_{i \geq j} a_i}  \leq
	\lceil \log
	(1/\eps) \rceil + 2.$$
\end{lemma}

\begin{proof}
For $i < N$, let $s_i = \sum_{j \geq i} a_j$;  clearly, $s_i$ is a
decreasing sequence and $s_{N-1} > \epsilon$.
%
Let $\ell_i$ be the largest index such that
$s_{\ell_i} = \sum_{j = \ell_i}^{N} a_j \geq \frac{1}{2^i}$.

By definition,
$$\sum_{j = \ell_i+1}^{\ell_{i+1}} a_j \leq \sum_{j = \ell_i+1}^{N} a_j
< \frac{1}{2^{i}} $$

Let $t = \lceil \log(1/\eps) \rceil$.
Clearly, $\ell_{t} \geq N-1$.
Now, we have,
\begin{align*}
	\sum_{i = 1}^{N-1} \frac{a_i}{s_i} &= \sum_{i = 0}^{t}
	\sum_{j = \ell_i + 1}^{\ell_{i+1}} \frac{a_j}{s_j} \\
	& \leq 	\sum_{i = 0}^{t}
	\frac{ \sum_{j = \ell_i + 1}^{\ell_{i+1}} a_j}{s_{\ell_{i+1}}} \\
	& \leq \sum_{i=0}^{t} 1  = t+1.
\end{align*}

\end{proof}

We have the following immediate consequence of the above lemma.

\begin{corollary} \label{cor:sumnode}
For every vertex $v$,
$$ \sum_{w \in C_v} \frac{\mu(w|v)}{\theta(w|v)} \leq
\lceil \log(1/\delta) \rceil +2. $$
\end{corollary}
\begin{proof}
Let $C_v = (w_1,\ldots,w_{c_v})$. Then, $\theta(w_{c_{v-1}} | v) = \mu(w_{c_{v-1}} | v ) + \mu(w_{c_v} | v) \geq \delta$. As $\theta(w_i | v) = \sum_{j \geq i} \mu(w_j | v)$, the claim now follows by applying the previous lemma to the numbers $\mu(w_1|v),\mu(w_2 | v),\ldots,\mu(w_{c_v} | v)$. 
\end{proof}


\begin{lemma}
	The sum over all leaves
	$$ \sum_{\text{ paths } v_1,w_1,\ldots, w_{\ell-1},v_\ell}
	q^{-|F_{v_\ell}|} \prod_{i = 1}^{\ell}
	\frac{\mu(w_i|v_i)}{\theta(w_i|v_i)} \leq \bkets{\lceil \log 1/\delta\rceil + 2}^{d}$$ \label{lem:path-estimate}
\end{lemma}
\begin{proof}
	For each $v$ corresponding to a \Dec call, define a probability distribution $\gamma(\;|v)$ over
	$C_v$ as follows: for each $w \in C_v$, $$\gamma(w|v) = \frac{\mu(w|v)}{\theta(w|v)} \cdot
	\left(\sum_{w \in C_v} \frac{\mu(w|v)}{\theta(w|v)} \right)^{-1}.$$ 
	
	For each $w$ corresponding to a $\XDec$ or $\YDec$ call consider the uniform distribution over the children of $w$. Then, these distributions induce a probability distribution over the leaves of the execution tree: the probability of any leaf $v_{\ell+1}$ is given by $\prod_{i = 1}^{\ell} q^{-|S_{w_i}|} \cdot
	\gamma(w_i|v_i)$, where $v_1,w_1,\ldots, v_\ell ,w_\ell, v_{\ell+1}$ is the path from the root to $v_{\ell+1}.$

By our construction, the total probability under the above distribution of all the leaves is $1.$ Thus, the sum over all leaves
$$ \sum_{\text{ paths } v_1,w_1,\ldots, v_\ell w_\ell}
	\prod_{i = 1}^{\ell} q^{-|S_{w_i}|} \cdot
	\gamma(w_i|v_i) = 1. $$

    By Corollary \ref{cor:sumnode}, $\gamma(w_i | v_i) \geq
	\frac{\mu(w_i|v_i)}{\theta(w_i|v_i)} \cdot
	\frac{1}{\bkets{\lceil \log 1/\delta\rceil + 2}} $.  The result follows from substituting this into the previous expression and using the fact that $\ell \leq d$ (number of fixed coordinates is at most $d$).
\end{proof}

We are now ready to bound $\mu(\Errorb)$.

\begin{lemma} $\mu(\Errorb) \leq q^{-0.1 d} \cdot 2^t  \cdot
	\bkets{\lceil \log 1/\delta\rceil + 2}^{d}$.\label{lem:proof-part-3}
\ignore{
	Suppose the distribution $\mu$ satisfies $H_{\infty}(\mu_{I}) \geq 1.9 \cdot \log q \cdot |I| - t$ then
		$$ \sum_{v_{d+1} \in Bad} \mu(v_{d+1}) \leq q^{-0.1 d} \cdot 2^t  \cdot
	\bkets{\lceil \log 1/\delta\rceil + 2}^{d}.
	$$ \label{lem:proof-part-3}}
\end{lemma}
\begin{proof}
Let \emph{Bad} denote all leaves that resulted in rectangles being added to $\Errorb$. The proof follows by using Lemmas \ref{lem:bad-path-prob} and Lemma \ref{lem:path-estimate}. For brevity, in the following, let $v_1,w_1,\ldots,v_\ell,w_\ell,v_{\ell+1} = v$ be the path to $v$ from the root. 
	\begin{align*}
		\sum_{v \in Bad} \mu(v) & \leq \sum_{v \in Bad} q^{-1.1 |F_{v}|} \cdot 2^t  \cdot \prod_{i=1}^{\ell} \frac{\mu(w_i|v_i)}{\theta(w_i | v_i)} \\
	%
	& \leq q^{-0.1d} \cdot 2^{t} \left(\sum_{v \in Bad} q^{- |F_{v}|}  \cdot \prod_{i=1}^{\ell} \frac{\mu(w_i|v_i)}{\theta(w_i | v_i)} \right)
%
	\leq q^{-0.1d} \cdot 2^{t} \cdot \bkets{\lceil \log 1/\delta\rceil + 2}^{d}.
\end{align*}
\end{proof}

\begin{proof}[Proof of \prettyref{thm:alg-analysis}]
One executing \prettyref{alg:dec}, we obtain a parition of $[q]^n \times [q]^n$ into $\cup_{v \in \cL} \cR(v) \cup \Error$, where we define $\Error = \Errora \cup \Errorb$. 

%On executing the algorithm in figure \prettyref{alg:dec}, the output consists of a sequence of rectangles $\{\cR_i\}_{i \in [N]}$ and a subset $\Error \subseteq [q]^n \times [q]^n$.  
	By \prettyref{lem:proof-part-1}, $\mu_{|\cR(v)}$ is an aligned $d$-\cbd for each $v \in \cL$.  Furthermore, the total measure of $\Error$ is 
\begin{align*}
	 \mu(\Error) & = \mu(\Errora) + \mu(\Errorb) \\
	 & \leq d\delta + q^{-0.1 d} \cdot 2^t  \cdot	\bkets{\lceil \log 1/\delta\rceil + 2}^{d} \mcom \qquad (\text{\prettyref{lem:proof-part-2} and \prettyref{lem:proof-part-3}})\\
	 & \leq  2^t \cdot (d q^{-0.05 })^d \qquad \qquad \qquad (\text{ for } \delta = q^{-0.05d}).
 \end{align*}
 This completes the proof.
\end{proof}














%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5




















\iffalse
\subsection{Applications}
We can complete the proof of Lemma \ref{lem:maindecomp} using \prettyref{thm:alg-analysis}.

\begin{proof}[Proof of \prettyref{lem:maindecomp}]
We let $\mu = pq$. Then, $H_{\infty}(\mu) \geq 2nb-t$. We run Algorithm \ref{alg:dec} on $\on^{bn} \times \on^{bn}$ with density $\mu$ and parameters $d = 40t/b$ and $\delta = 2^{-t}.$

We let $E$ be the density $\mu_{\mid \Errora \cup \Errorb}$ and for each $i$, let $\nu_i$ be the density $\mu_{\mid R_i}$ and let $\lambda_i = \mu(R_i) \geq 0 $ and $\lambda_{err} = \mu(E) \geq 0.$ Then, since $R_1, R_2, \ldots, R_q,\Errora, \Errorb$ is a partition of $\on^{bn} \times \on^{bn}$ we have: $$\mu = \sum_{i = 1}^q \lambda_i \mu_{\mid R_i} + \lambda_{err} \mu_{\mid E},$$ and $\sum_{i = 1}^q \lambda_i + \lambda_{err} = 1.$

Each $\nu_i$ is $d$-$\cbd$ from claim 1 of \prettyref{thm:alg-analysis}. The last two claims of \prettyref{thm:alg-analysis} can now be used to  bound $\lambda_{err}$:

$$\lambda_{err} \leq d 2^{-t} + 2^{-0.1Ct} 2^{t} 2^{Ct/b \log{(t+2)}}.$$

Now, $\log{(t)} \leq 2 \log{(n)}$ for any $b < n.$ Choose $C = 40$ and we know that $n > b > 80 \log{(n)}.$ Then, the second term above evaluates to at most $2^{-2t}.$ The first term is at most $2^{-t}.$ Thus the $\lambda_{err} < 2^{-t}$ as required.

\end{proof}



\subsubsection{Decomposition Theorem and Proof of Lemma \ref{lem:mainjunta-restated}}
%
%For our applications, however, we need a significantly strengthened statement that gains from having a product of two high min-entropy random variables.  Our main decompositi%on lemma states that up to some small error any pair of high min-entropy distributions $u,v$ on $[q]^{n}$ can be decomposed into a convex combination of \emph{aligned $d$-\cbd} %distributions.


\begin{lemma}\label{lem:maindecomp}
%Let $b \geq \alpha_1 \log{(n)}$ for some large enough constant $\alpha_1$.
Let $u_0, v_0$ be densities on $[q]^{n}$ satisfying $H_{\infty}(u_0) + H_{\infty}(v_0) \geq (2n - t) \cdot \log q$ for some $t > 0.$ Then, for all $d \geq 40 t$ and $\log q > 80 \log_2{(n)}$, there exists densities $\nu_i$ such that $u_0v_0 = \sum_{i=1}^N \lambda_i \nu_i + \lambda_{err} E$ such that
\begin{itemize}
\item for every $1 \leq i \leq N$, $\nu_i$ is an aligned $d$-\cbd density.
%\item $\nu_i$ is a density supported on some rectangle $X_i \times Y_i \on^{bn} \times \on^{bn}$ ,
\item $0 \leq \lambda_i, \lambda_{err} \leq 1$, $\sum_{i=1}^N \lambda_i + \lambda_{err} = 1$,
\item $|\lambda_{err}| < 2^{-t}$, and
\end{itemize}
\end{lemma}

%It is tempting to attempt to prove this lemma by individually decomposing each of the two high min-entropy densities separately, and then taking their product . However, it i%s unclear how to simultaneously ensure the property of each of the pieces in the decomposition being \emph{aligned} and at the same time, having the error decrease exponentia%lly in the entropy gap $t$. Having both these properties together is crucial to our proof.

It is easy to complete the proof of Theorem \ref{lem:mainjunta-restated} using Lemma \ref{lem:junta-approx-for-CBD} and Lemma \ref{lem:maindecomp}.

\begin{proof}[Proof of Theorem \ref{lem:mainjunta-restated}]

Recall that $A_{u,v}(z)  = \E[ \1_z(x,y) u(x)v(y)]$ where $z$ is the $2^n$ scaled $0$-$1$ indicator of $\{(x,y) \mid \iproduct^{\otimes n}(x,y) = z\}.$  Apply Lemma \ref{lem:maindecomp} to $u$ and $v$. Let $X_i, Y_i, \lambda_i, \nu_i$ for $1 \leq i \leq N$ and $\lambda_err,E$ be the output parameters of the decomposition of $pq.$

Then, $A_{u,v}(z) = \sum_{i = 1}^N \lambda_i \E[ \1_z(x,y) \nu_i(x,y)] + \lambda_{err} \E_{(x,y) \sim E}[ \1_z(x,y) E(x,y)].$ Let $\delta$ be the density induced on $\on^{n}$ by $E$,i.e., $\delta(z) = \E[ \1_z(x,y) E(x,y)].$

Observe that $\E[\1_z(x,y) \nu_i(x,y)]$ is just the density of $\iproduct^{\otimes n }(X_i,Y_i)$ and since $(X_i, Y_i)$ are aligned $d$-CBD, using Lemma  \ref{lem:junta-approx-for-CBD} we obtain for each $1 \leq i \leq N$,  non-negative $d$-conjunctions $J_i$, coefficients $C_i$ and $\epsilon$-decaying functions $h_i$ for $\epsilon = 2^{-0.5b}$ such that $\E[ \1_z(x,y) \nu_i(x,y)] = C_i J_i(z) (1+h_i(z)).$

This completes the proof.
\end{proof}

\fi


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5








